Testing for the Minimum Mean-Variance Spanning Set

This paper explores the estimation and inference of the minimum spanning set (MSS), the smallest subset of risky assets that spans the mean-variance efficient frontier of the full asset set. We establish identification conditions for the MSS and develop a novel procedure for its estimation and inference. Our theoretical analysis shows that the proposed MSS estimator covers the true MSS with probability approaching 1 and converges asymptotically to the true MSS at any desired confidence level, such as 0.95 or 0.99. Monte Carlo simulations confirm the strong finite-sample performance of the MSS estimator. We apply our method to evaluate the relative importance of individual stock momentum and factor momentum strategies, along with a set of well-established stock return factors. The empirical results highlight factor momentum, along with several stock momentum and return factors, as key drivers of mean-variance efficiency. Furthermore, our analysis uncovers the sources of contribution from these factors and provides a ranking of their relative importance, offering new insights into their roles in mean-variance analysis.

==> sa.tex <==
%2multibyte Version: 5.50.0.2890 CodePage: 936
%TCIDATA{Version=5.50.0.2890}
%TCIDATA{Codepage=936}
%TCIDATA{LaTeXparent=0,0,MSS_Main.tex}
                      

\section{Proof of Lemmas in Section \protect \ref{AP: AU_L} \label{SAP:
Pf_AUL}}

In this appendix, we present the proofs of the lemmas provided in Section %
\ref{AP: AU_L} of the paper. Auxiliary results used in these proofs are
included in the subsequent appendix.

Throughout both appendices, we maintain the same notation as in the main
text. Additional notation introduced specifically for the proofs below is
described as follows: we use $\lambda _{\min }(A)$ and $\lambda _{\max }(A)$
to represent the smallest and largest eigenvalues, respectively, of any real
symmetric matrix $A$. The notation $\left \Vert \cdot \right \Vert $ refers
to the matrix Frobenius norm, while $\left \Vert \cdot \right \Vert _{q}$
represents the $L_{q}$ norm of a random variable. Let $\mathrm{P}^{\ast
}(\cdot )$\ denote the probability conditional on the data.\ Similarly, $%
\mathrm{E}^{\ast }[\cdot ]$,\ $\mathrm{Var}^{\ast }(\cdot )$ and $\mathrm{Cov%
}^{\ast }(\cdot )$ denote expectation, variance and covariance,
respectively, taken under $\mathrm{P}^{\ast }(\cdot )$ given the data.
Recall that $C$ is used to indicate a positive constant that is independent
of $i$, $t$ and $T$, and its value may vary across different lines.

\bigskip

\noindent \textsc{Proof of Lemma \ref{OLS_Coff}.}\ Let $I_{d,-i}$ denote the
submatrix of $I_{d}$ without its $i$-th column. Then 
\begin{equation*}
(\ell _{d,i},I_{d,-i})^{\top }\Sigma (\ell _{d,i},I_{d,-i})=\mathrm{Var}%
((R_{i},R_{-i}^{\top })^{\top }),
\end{equation*}%
which implies: 
\begin{eqnarray}
\ell _{d,i}^{\top }\Sigma ^{-1} &=&\ell _{d,i}^{\top }(\ell
_{d,i},I_{d,-i})((\ell _{d,i},I_{d,-i})^{\top }\Sigma (\ell
_{d,i},I_{d,-i}))^{-1}(\ell _{d,i},I_{d,-i})^{\top }  \notag \\
&=&\ell _{d,1}^{\top }(\mathrm{Var}((R_{i},R_{-i}^{\top })^{\top
}))^{-1}(\ell _{d,i},I_{d,-i})^{\top }.  \label{P_OLS_Coff_1}
\end{eqnarray}%
Using the block matrix inversion formula:%
\begin{equation}
(\mathrm{Var}((R_{i},R_{-i}^{\top })^{\top }))^{-1}=\left( 
\begin{array}{cc}
\tilde{\sigma}_{i}^{-2} & -\frac{\Gamma _{i,-i}\Sigma _{-i}^{-1}}{\tilde{%
\sigma}_{i}^{2}} \\ 
-\frac{\Sigma _{-i}^{-1}\Gamma _{i,-i}^{\top }}{\tilde{\sigma}_{i}^{2}} & 
\tilde{\Sigma}_{-i}^{-1}%
\end{array}%
\right) ,  \label{P_OLS_Coff_2}
\end{equation}%
where $\tilde{\Sigma}_{-i}\equiv \Sigma _{-i}-\sigma _{i}^{-2}\Gamma
_{i,-i}^{\top }\Gamma _{i,-i}$. Since $\Sigma $ is non-singular, it is
strictly positive definite, and so is its inverse $\Sigma ^{-1}$. The
diagonal elements of $\Sigma ^{-1}$ are $\tilde{\sigma}_{i}^{-2}$, which
ensures $\tilde{\sigma}_{i}^{2}>0$. Combining these results, we find:%
\begin{equation}
\ell _{d,i}^{\top }\Sigma ^{-1}=\tilde{\sigma}_{i}^{-2}\left( 
\begin{array}{cc}
1 & -\Gamma _{i,-i}\Sigma _{-i}^{-1}%
\end{array}%
\right) (\ell _{d,i},I_{d,-i})^{\top }.  \label{P_OLS_Coff_3}
\end{equation}%
Thus 
\begin{equation}
\ell _{d,i}^{\top }\Sigma ^{-1}\mu =\tilde{\sigma}_{i}^{-2}\left( 
\begin{array}{cc}
1 & -\Gamma _{i,-i}\Sigma _{-i}^{-1}%
\end{array}%
\right) \left( 
\begin{array}{c}
\mu _{i} \\ 
\mu _{-i}%
\end{array}%
\right) =\tilde{\sigma}_{i}^{-2}(\mu _{i}-\Gamma _{i,-i}\Sigma _{-i}^{-1}\mu
_{-i}).  \label{P_OLS_Coff_4}
\end{equation}%
Similarly: 
\begin{equation}
\ell _{d,i}^{\top }\Sigma ^{-1}1_{d}=\tilde{\sigma}_{i}^{-2}\left( 
\begin{array}{cc}
1 & -\Gamma _{i,-i}\Sigma _{-i}^{-1}%
\end{array}%
\right) 1_{d}=\tilde{\sigma}_{i}^{-2}(1-\Gamma _{i,-i}\Sigma
_{-i}^{-1}1_{d-1}).  \label{P_OLS_Coff_5}
\end{equation}%
From the formula for LS regression,\ the coefficients $\alpha _{i}$ and\ $%
\beta _{i}$\ in (\ref{ID_1}) satisfy: 
\begin{equation}
\alpha _{i}=\mu _{i}-\mu _{-i}^{\top }\beta _{i}\  \  \text{and}\  \  \beta
_{i}=\Sigma _{-i}^{-1}\Gamma _{i,-i}^{\top }.  \label{P_OLS_Coff_6}
\end{equation}%
Combining these expressions with the results derived above completes the
proof of the lemma.\hfill $Q.E.D.$

\bigskip

\noindent \textsc{Proof of Lemma \ref{I_L1b}.} Since $\hat{\varepsilon}%
_{i,t}=$ $R_{i,t}-\hat{\alpha}_{i}-R_{-i,t}^{\top }\hat{\beta}%
_{i}=\varepsilon _{i,t}-(\hat{\alpha}_{i}-\alpha _{i})-R_{-i,t}^{\top }(\hat{%
\beta}_{i}-\beta _{i})$,\ we can write:%
\begin{eqnarray}
T^{-1}\sum_{t\leq T}\hat{\varepsilon}_{i,t}^{2} &=&T^{-1}\sum_{t\leq
T}\varepsilon _{i,t}^{2}-2(\hat{\alpha}_{i}-\alpha _{i},\hat{\beta}%
_{i}^{\top }-\beta _{i}^{\top })^{\top }T^{-1}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}  \notag \\
&&+(\hat{\alpha}_{i}-\alpha _{i},\hat{\beta}_{i}^{\top }-\beta _{i}^{\top
})^{\top }\hat{Q}_{-i}(\hat{\alpha}_{i}-\alpha _{i},\hat{\beta}_{i}^{\top
}-\beta _{i}^{\top }).  \label{P_I_L1_13}
\end{eqnarray}%
By Lemma \ref{I_L1}(ii, iii) and (\ref{P_I_L1_12}), the last two terms on
the right-hand side of equation\ (\ref{P_I_L1_13}) can be bounded as: 
\begin{equation}
\max_{i\leq d}\left \vert (\hat{\alpha}_{i}-\alpha _{i},\hat{\beta}%
_{i}^{\top }-\beta _{i}^{\top })^{\top }T^{-1}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}\right \vert =O_{p}(T^{-1})  \label{P_I_L1_14}
\end{equation}%
and 
\begin{equation}
\max_{i\leq d}(\hat{\alpha}_{i}-\alpha _{i},\hat{\beta}_{i}^{\top }-\beta
_{i}^{\top })^{\top }\hat{Q}_{-i}(\hat{\alpha}_{i}-\alpha _{i},\hat{\beta}%
_{i}^{\top }-\beta _{i}^{\top })=O_{p}(T^{-1}),  \label{P_I_L1_15}
\end{equation}%
respectively. By Assumption \ref{A1}(ii) and (\ref{P_I_L1_6}), we have%
\begin{equation}
\max_{i\leq d}\mathrm{E}\left[ |\varepsilon _{i,t}|^{r}\right] \leq
C\max_{i\leq d}\mathrm{E}\left[ |R_{i,t}-\mu _{i}|^{r}+|(R_{-i,t}-\mu
_{-i})^{\top }\beta _{i}|^{r}\right] \leq C\sum_{i\leq d}\mathrm{E}\left[
|R_{i,t}-\mu _{i}|^{r}\right] \leq C.  \label{P_I_L1_15b}
\end{equation}%
Therefore, using arguments similar to those for deriving (\ref{P_I_L1_1b}),
we obtain 
\begin{equation*}
\max_{i\leq d}\mathrm{E}\left[ \left \vert T^{-1/2}\sum_{t\leq
T}(\varepsilon _{i,t}^{2}-\sigma _{\varepsilon _{i}}^{2})\right \vert ^{2}%
\right] \leq C+2T^{-1}\sum_{t=2}^{T}\sum_{s=1}^{t-1}\alpha
_{t-s}^{1-4/r}\left \Vert \varepsilon _{i,t}\right \Vert _{r}^{2}\left \Vert
\varepsilon _{i,s}\right \Vert _{r}^{2}\leq C,
\end{equation*}%
which, along with Markov's inequality, implies 
\begin{equation}
\max_{i\leq d}\left \vert T^{-1}\sum_{t\leq T}(\varepsilon _{i,t}^{2}-\sigma
_{\varepsilon _{i}}^{2})\right \vert =O_{p}(T^{-1/2}).  \label{P_I_L1_16}
\end{equation}%
Collecting the results in (\ref{P_I_L1_13}), (\ref{P_I_L1_14}), (\ref%
{P_I_L1_15}) and (\ref{P_I_L1_16}), we conclude: 
\begin{equation}
\max_{i\leq d}\left \vert \hat{\sigma}_{\varepsilon _{i}}^{2}-\sigma
_{\varepsilon _{i}}^{2}\right \vert =O_{p}(T^{-1/2}).  \label{P_I_L1_17}
\end{equation}%
Moreover by Assumption \ref{A1}(iii), 
\begin{equation}
\min_{i\leq d}\sigma _{\varepsilon _{i}}^{2}\geq \lambda _{\min }(Q)>C.
\label{P_I_L1_18}
\end{equation}%
By the definition of $\hat{s}_{i,j}^{2}$, we have 
\begin{eqnarray*}
\max_{i\leq d}\max_{j=1,2}\frac{\left \vert \hat{s}_{i,j}^{2}-s_{i,j}^{2}%
\right \vert }{s_{i,j}^{2}} &\leq &\max_{i\leq d}\max_{j=1,2}\left( \frac{%
\left \vert (\hat{\sigma}_{\varepsilon _{i}}^{2}-\sigma _{\varepsilon
_{i}}^{2})A_{j,\cdot }\hat{Q}_{-i}^{-1}A_{j,\cdot }^{\top }\right \vert }{%
\sigma _{\varepsilon _{i}}^{2}A_{j,\cdot }Q_{-i}^{-1}A_{j,\cdot }^{\top }}+%
\frac{\left \vert A_{j,\cdot }(\hat{Q}_{-i}^{-1}-Q_{-i}^{-1})A_{j,\cdot
}^{\top }\right \vert }{A_{j,\cdot }Q_{-i}^{-1}A_{j,\cdot }^{\top }}\right)
\\
&\leq &\max_{i\leq d}\max_{j=1,2}\left( \frac{\lambda _{\max }(Q_{-i})\left
\vert \hat{\sigma}_{\varepsilon _{i}}^{2}-\sigma _{\varepsilon
_{i}}^{2}\right \vert }{\sigma _{\varepsilon _{i}}^{2}\lambda _{\min }(\hat{Q%
}_{-i})}+\frac{\lambda _{\max }(Q_{-i})\left \Vert \hat{Q}_{-i}-Q_{-i}\right
\Vert }{\lambda _{\min }(\hat{Q}_{-i})\lambda _{\min }(Q_{-i})}\right) \\
&=&O_{p}(T^{-1/2}),
\end{eqnarray*}%
where the equality is by (\ref{P_I_L1_17}), (\ref{P_I_L1_18}), (\ref%
{P_I_L1_5}), (\ref{P_I_L1_12}) and Lemma \ref{I_L1}(i).\hfill $Q.E.D.$

\bigskip

\noindent \textsc{Proof of Lemma \ref{I_L3}.} By the definition of $e_{t}$,
we can express 
\begin{equation}
\left( \left( \frac{A_{j,\cdot }Q_{-i}^{-1}T^{-1/2}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}}{s_{i,j}}\right) _{j=1,2}\right) _{i\leq d}=%
\mathrm{diag}\left( ((s_{i,j}^{-1})_{j=1,2})_{i\leq d}\right)
T^{-1/2}\sum_{t\leq T}e_{t}.  \label{P_I_L3_1}
\end{equation}%
Thus, it is sufficient to show that%
\begin{equation}
T^{-1/2}\sum_{t\leq T}e_{t}\rightarrow _{d}N(0,\Omega _{d}),
\label{P_I_L3_2}
\end{equation}%
since the claim of the lemma follows from (\ref{P_I_L3_2}), Lemma \ref{I_L2}
and the continuous mapping theorem.

By Assumption \ref{A1}(ii) and (\ref{P_I_L1_6}), for any $i,i^{\prime }\leq
d $ with $i^{\prime }\neq i$, we apply H\"{o}lder's inequality to obtain:%
\begin{equation}
\mathrm{E}\left[ |R_{i^{\prime },t}(R_{i,t}-\mu _{i})|^{r/2}\right] \leq C%
\text{ \ and \ }\mathrm{E}\left[ |R_{i^{\prime },t}(R_{-i,t}-\mu
_{-i})^{\top }\beta _{i}|^{r/2}\right] \leq C.  \label{P_I_L3_3}
\end{equation}%
Since $\varepsilon _{i,t}=(R_{i,t}-\mu _{i})-(R_{-i,t}-\mu _{-i})^{\top
}\beta _{i}$, by (\ref{P_I_L3_3}), we deduce that: 
\begin{equation}
\mathrm{E}\left[ |R_{i^{\prime },t}\varepsilon _{i,t}|^{r/2}\right] \leq C.
\label{P_I_L3_4}
\end{equation}%
By H\"{o}lder's inequality\ and\ the Cauchy-Schwarz inequality,\ we have 
\begin{equation}
\mathrm{E}\left[ ||e_{t}||^{r/2}\right] \leq C\sum_{i\leq d}\mathrm{E}\left[
||e_{i,t}||^{r/2}\right] \leq C\sum_{i\leq d}\mathrm{E}\left[ \left \vert |%
\tilde{R}_{-i,t}\varepsilon _{i,t}|\right \vert ^{r/2}\right] \leq C,
\label{P_I_L3_5}
\end{equation}%
where the last inequality follows from (\ref{P_I_L1_15b}) and (\ref{P_I_L3_4}%
). Since $\left \{ e_{t}\right \} _{t}$ is a strictly stationary and strong
mixing process with mixing coefficient $\alpha _{j}$ and $\sum_{j=0}\alpha
_{j}^{1-4/r}<C$ by Assumption \ref{A1}(i),\ we can use (\ref{P_I_L3_5}) to
invoke the central limit theorem for strong mixing processes, see, e.g.,\
Theorem 14.15 in \cite{hansen2022} to establish (\ref{P_I_L3_2}).\hfill $%
Q.E.D.$

\bigskip

\noindent \textsc{Proof of Lemma \ref{B_L7a}.} Under the subset of the
sampling space\ $\mathcal{D}_{4,T}$ (which is defined before Lemma \ref{B_L5}
below), we can apply Lemma \ref{B_L5a} to obtain%
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \left \vert \max_{i\leq d}M_{i,T}^{b}-\max_{i\leq
d}\tilde{M}_{i,T}^{b}\right \vert \geq \ell ^{c_{6}}T^{-2c_{6}+1/2}\right)  
\notag \\
&\leq &C\max_{i\leq d}\max_{j=1,2}\mathrm{P}^{\ast }\left( \left \vert \frac{%
T^{1/2}(\hat{\theta}_{i,j}^{b}-\hat{\theta}_{i,j})}{\hat{s}_{i,j}^{b}}-\frac{%
(m\ell )^{-1/2}\sum_{t\leq m\ell }e_{i,j,t}^{b}}{s_{i,j}}\right \vert \geq
\ell ^{c_{6}}T^{-2c_{6}+1/2}\right)   \notag \\
&\leq &C(\ell T^{-1})^{1-2c_{6}},  \label{P_B_L7a_1}
\end{eqnarray}%
for any $c_{6}\in (1/3,1/2)$.\ Therefore for any $\tilde{C}_{0}>0$, 
\begin{eqnarray}
\mathrm{P}^{\ast }\left( \max_{i\leq d}M_{i,T}^{b}\geq \tilde{C}_{0}\right) 
&\leq &\mathrm{P}^{\ast }\left( \max_{i\leq d}\tilde{M}_{i,T}^{b}\geq \tilde{%
C}_{0}/2\right) +C(\ell T^{-1})^{1-2c_{6}}  \notag \\
&\leq &C\tilde{C}_{0}^{-2}\mathrm{Var}^{\ast }\left( (m\ell
)^{-1/2}\sum_{t\leq m\ell }e_{i,j,t}^{b}\right) +C(\ell T^{-1})^{1-2c_{6}} 
\notag \\
&\leq &C\tilde{C}_{0}^{-2}+C(\ell T^{-1})^{1-2c_{6}},  \label{P_B_L7a_2}
\end{eqnarray}%
where the second inequality is by Markov's inequality,\ (\ref{P_I_L1_18})\
and\ (\ref{P_I_L1_5}), the last inequality is by\ (\ref{P_I_L1_5}) and\ (\ref%
{D_2T_2}). We can choose a sufficiently large value for $\tilde{C}_{0}$,
denoted as $\tilde{C}_{p}$, such that $C\tilde{C}_{p}^{-2}+C(\ell
T^{-1})^{1-2c_{6}}\leq p$ for sufficiently large $T$.\ This, combined with (%
\ref{P_B_L7a_2}), shows that 
\begin{equation*}
\mathrm{P}^{\ast }\left( \max_{i\leq d}M_{i,T}^{b}\geq \tilde{C}_{p}\right)
\leq p
\end{equation*}%
and $cv_{1-p,T}^{b}(\mathcal{M}_{d})\leq \tilde{C}_{p}$ under $\mathcal{D}%
_{4,T}$. Since\ $\mathrm{P}\left( \mathcal{D}_{4,T}\right) \rightarrow 1$ as 
$T\rightarrow \infty $, it follows that $cv_{1-p,T}^{b}(\mathcal{M}%
_{d})=O_{p}(1)$.\hfill $Q.E.D.$

\bigskip

\noindent \textsc{Proof of Lemma \ref{B_L7}.}\ Let $\xi _{i,j}^{\ast }$
denote the $j$-th entry of $(\ell _{d,i}^{\top }\otimes \mathrm{diag}%
(s_{i,1}^{-1},s_{i,2}^{-1}))(\Omega _{T}^{\ast })^{1/2}\mathcal{N}_{d}$ For
any $i\leq d$ and $j=1,2$, where $\Omega _{T}^{\ast }\equiv \mathrm{Var}%
^{\ast }((m\ell )^{-1/2}\sum_{t\leq m\ell }e_{t}^{b})$, $e_{t}^{b}\equiv
(e_{i,t}^{b})_{i\leq d}$ and $e_{i,t}^{b}\equiv (e_{i,j,t}^{b})_{j=1,2}$. By
Lemma \ref{B_L6}, we have:%
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \left \vert \max_{i\notin \mathcal{S}}\tilde{M}%
_{i,T}^{b}-\max_{i\notin \mathcal{S}}\tilde{M}_{i}^{\ast }\right \vert \geq
\log (T)^{-2/3}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}\max_{j=1,2}\frac{%
\left \vert (m\ell )^{-1/2}\sum_{t\leq m\ell }e_{i,j,t}^{b}-s_{i,j}\xi
_{i,j}^{\ast }\right \vert }{s_{i,j}}\geq \log (T)^{-2/3}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert (m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{t}^{b}-(\Omega _{T}^{\ast })^{1/2}\mathcal{N}_{d}\right \Vert \geq
\min_{i\leq d}\min_{j=1,2}s_{i,j}\log (T)^{-2/3}\right)  \notag \\
&\leq &C\log (T)^{5/2}(\ell T^{-1})^{1/2},  \label{P_B_L7_0}
\end{eqnarray}%
where $\tilde{M}_{i}^{\ast }\equiv \left \Vert (\ell _{d,i}^{\top }\otimes 
\mathrm{diag}(s_{i,1}^{-1},s_{i,2}^{-1}))(\Omega _{T}^{\ast })^{1/2}\mathcal{%
N}_{d}\right \Vert _{\infty }$. Therefore, conditional on $\mathcal{D}_{4,T}$%
, it follows that for sufficiently large $T$: 
\begin{eqnarray}
\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}M_{i,T}^{b}\geq x\right)
&\leq &\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}\tilde{M}%
_{i,T}^{b}\geq x-\log (T)^{-2/3}\right) +o(\log (T)^{-1})  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}\tilde{M}%
_{i}^{\ast }\geq x-2\log (T)^{-2/3}\right) +o(\log (T)^{-1})  \notag \\
&\leq &\mathrm{P}\left( \max_{i\notin \mathcal{S}}\tilde{M}_{i}\geq x-2\log
(T)^{-2/3}\right) +o(\log (T)^{-1/4})  \notag \\
&\leq &\mathrm{P}\left( \max_{i\notin \mathcal{S}}\tilde{M}_{i}\geq x\right)
+\log (T)^{-1/4},  \label{P_B_L7_1}
\end{eqnarray}%
where the first inequality is by Lemmas \ref{B_L5a}, the second inequality
follows from (\ref{P_B_L7_0}), the third and the last inequality follow from
Lemmas \ref{B_L6b} and \ref{Para_Anti}, respectively. Letting $%
x=cv_{1-p+\delta _{T}}^{u}(\mathcal{S})$ with $\delta _{T}=\log (T)^{-1/4}$
in (\ref{P_B_L7_1}) obtains%
\begin{equation}
\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}M_{i,T}^{b}\geq
cv_{1-p+\delta _{T}}^{u}(\mathcal{S})\right) \leq \mathrm{P}\left(
\max_{i\notin \mathcal{S}}\tilde{M}_{i}\geq cv_{1-p+\delta _{T}}^{u}(%
\mathcal{S})\right) +\delta _{T}\leq p,  \label{P_B_L7_2}
\end{equation}%
where the second inequality is by the definition of $cv_{1-p+\delta
_{T}}^{u}(\mathcal{S})$. This shows that $cv_{1-p,T}^{b}(\mathcal{S})\leq
cv_{1-p+\delta _{T}}^{u}(\mathcal{S})$ wpa1.

Similarly, conditioning on $\mathcal{D}_{4,T}$\ we have for any $x\geq 0$
and all large $T$, 
\begin{eqnarray}
\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}M_{i,T}^{b}\geq x\right)
&\geq &\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}\tilde{M}%
_{i,T}^{b}\geq x+\log (T)^{-2/3}\right) -o(\log (T)^{-1})  \notag \\
&\geq &\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}\tilde{M}%
_{i}^{\ast }\geq x+2\log (T)^{-2/3}\right) -o(\log (T)^{-1})  \notag \\
&\geq &\mathrm{P}\left( \max_{i\notin \mathcal{S}}\tilde{M}_{i}\geq x+2\log
(T)^{-2/3}\right) -o(\log (T)^{-1/4})  \notag \\
&\geq &\mathrm{P}\left( \max_{i\notin \mathcal{S}}\tilde{M}_{i}\geq x\right)
-\log (T)^{-1/4},  \label{P_B_L7_3}
\end{eqnarray}%
where the first inequality is by Lemma \ref{B_L5a}, the second inequality
follows from (\ref{P_B_L7_0}), the third and the last inequality follow from
Lemmas \ref{B_L6b} and \ref{Para_Anti}, respectively. Letting $%
x=cv_{1-p,T}^{b}(\mathcal{S})$ in (\ref{P_B_L7_3}) obtains 
\begin{equation*}
\mathrm{P}^{\ast }\left( \max_{i\notin \mathcal{S}}M_{i,T}^{b}\geq
cv_{1-p,T}^{b}(\mathcal{S})\right) \geq \mathrm{P}\left( \max_{i\notin 
\mathcal{S}}\tilde{M}_{i}\geq cv_{1-p,T}^{b}(\mathcal{S})\right) -\delta
_{T},
\end{equation*}%
which together with the definition of $cv_{1-p,T}^{b}(\mathcal{S})$ shows
that conditioning on $\mathcal{D}_{4,T}$%
\begin{equation}
\mathrm{P}\left( \max_{i\notin \mathcal{S}}\tilde{M}_{i}\geq cv_{1-p,T}^{b}(%
\mathcal{S})\right) \leq p+\delta _{T}.  \label{P_A_L6_5}
\end{equation}%
Therefore, we have $cv_{1-p,T}^{b}(\mathcal{S})\geq cv_{1-p-\delta _{T}}^{u}(%
\mathcal{S})$ wpa1.\hfill $Q.E.D.$

\bigskip

\noindent \textsc{Proof of Lemma\  \ref{T1}.}\ By the definition of $\widehat{%
\mathrm{MSS}}_{p,j}$ ($j=0,\ldots ,j^{\ast }$) and using (\ref{P_T1_0}), we
have 
\begin{equation}
cv_{1-p,T}^{b}(\mathcal{M}_{d}\backslash \widehat{\mathrm{MSS}}_{p,j})\leq
cv_{1-p,T}^{b}(\mathcal{M}_{d}\backslash \widehat{\mathrm{MSS}}_{p,j-1})%
\text{ \  \  \ and \  \  \ }\widehat{\mathrm{MSS}}_{p,j-1}\subseteq \widehat{%
\mathrm{MSS}}_{p,j}.  \label{P_T1_1}
\end{equation}%
Since $\widehat{\mathrm{MSS}}_{p,0}=\varnothing $, this result implies that
if $\widehat{\mathrm{MSS}}_{p}\nsubseteq \mathrm{MSS}$, there must exist a
smallest index $j^{\prime }$ for which $\widehat{\mathrm{MSS}}_{p,j^{\prime
}}\nsubseteq \mathrm{MSS}$. Consequently, the event $\widehat{\mathrm{MSS}}%
_{p}\nsubseteq \mathrm{MSS}$ implies 
\begin{equation}
\max_{i\in \mathrm{MSS}^{c}}M_{i,T}\geq cv_{1-p,T}^{b}(\mathcal{M}%
_{d}\backslash \widehat{\mathrm{MSS}}_{p,j^{\prime }-1})\text{ \  \  \  \ and \
\  \  \ }\widehat{\mathrm{MSS}}_{p,j^{\prime }-1}\subseteq \mathrm{MSS}\text{,}
\label{P_T1_2}
\end{equation}%
where $\mathrm{MSS}^{c}\equiv \mathcal{M}_{d}\backslash \mathrm{MSS}$.
Combining this result with (\ref{P_T1_0}), we obtain%
\begin{eqnarray}
\mathrm{P}\left( \widehat{\mathrm{MSS}}_{p}\nsubseteq \mathrm{MSS}\right) 
&\leq &\mathrm{P}\left( \max_{i\in \mathrm{MSS}^{c}}M_{i,T}\geq
cv_{1-p,T}^{b}(\mathcal{M}_{d}\backslash \widehat{\mathrm{MSS}}_{p,j^{\prime
}-1})\bigcap \widehat{\mathrm{MSS}}_{p,j^{\prime }-1}\subseteq \mathrm{MSS}%
\right)   \notag \\
&\leq &\mathrm{P}\left( \max_{i\in \mathrm{MSS}^{c}}M_{i,T}\geq
cv_{1-p,T}^{b}(\mathrm{MSS}^{c})\right) .  \label{P_T1_3}
\end{eqnarray}%
For any $p\in (0,1)$ and any $\mathcal{S}\subseteq \mathcal{M}_{d}$, let $%
cv_{1-p}^{u}(\mathcal{S})$ denote the ($1-p$)th quantile of $\max_{i\in 
\mathcal{S}}\tilde{M}_{i}$. Then, by Lemma \ref{B_L7}, there exists a
positive sequence $\delta _{T}=o(1)$ such that%
\begin{equation}
\mathrm{P}\left( \max_{i\in \mathrm{MSS}^{c}}M_{i,T}\geq cv_{1-p,T}^{b}(%
\mathrm{MSS}^{c})\right) \leq \mathrm{P}\left( \max_{i\in \mathrm{MSS}%
^{c}}M_{i,T}\geq cv_{1-p-\delta _{T}}^{u}(\mathrm{MSS}^{c})\right) +o(1).
\label{P_T1_4}
\end{equation}%
Hence, for any $\varepsilon \in (0,1-p)$, we have 
\begin{equation}
\mathrm{P}\left( \max_{i\in \mathrm{MSS}^{c}}M_{i,T}\geq cv_{1-p,T}^{b}(%
\mathrm{MSS}^{c})\right) \leq \mathrm{P}\left( \max_{i\in \mathrm{MSS}%
^{c}}M_{i,T}\geq cv_{1-p-\varepsilon }^{u}(\mathrm{MSS}^{c})\right) +o(1),
\label{P_T1_5}
\end{equation}%
for sufficiently large $T$. By Lemma \ref{I_L3}, it follows that 
\begin{equation}
\lim_{T\rightarrow \infty }\mathrm{P}\left( \max_{i\in \mathrm{MSS}%
^{c}}M_{i,T}\geq cv_{1-p-\varepsilon }^{u}(\mathrm{MSS}^{c})\right) =\mathrm{%
P}\left( \max_{i\in \mathrm{MSS}^{c}}\tilde{M}_{i}\geq cv_{1-p-\varepsilon
}^{u}(\mathrm{MSS}^{c})\right) .  \label{P_T1_6}
\end{equation}%
This, combined with (\ref{P_T1_3}), (\ref{P_T1_5}) and the definition of $%
cv_{1-p-\varepsilon }^{u}(\mathrm{MSS}^{c})$, shows that 
\begin{equation}
\underset{T\rightarrow \infty }{\lim \sup }\mathrm{P}\left( \widehat{\mathrm{%
MSS}}_{p}\nsubseteq \mathrm{MSS}\right) \leq p+\varepsilon .  \label{P_T1_7}
\end{equation}%
Since $\varepsilon $ is arbitrary, the claim of the lemma follows directly
from (\ref{P_T1_7}).\hfill $Q.E.D.$

\section{Auxiliary Results \label{SAP:AUR}}

\begin{lemma}
\label{I_L1} Under Assumption \ref{A1}, we have:

(i) $\hat{Q}-Q=O_{p}(T^{-1/2})$, where $\hat{Q}\equiv T^{-1}\sum_{t\leq T}%
\tilde{R}_{t}\tilde{R}_{t}^{\top }$;

(ii)\ $\max_{i\leq d}\left \Vert T^{-1/2}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}\right \Vert =O_{p}(1)$;

(iii) $\max_{i\leq d}||\hat{\theta}_{i}-\theta _{i}||^{2}=O_{p}(T^{-1})$.
\end{lemma}

\noindent \textsc{Proof.} (i)\ By the definition of $\hat{Q}$, and since $d$
is a fixed integer,\ it is sufficient to show that for any $i,i^{\prime
}\leq d$: 
\begin{equation}
T^{-1}\sum_{t\leq T}(R_{i,t}-\mu _{i})=O_{p}(T^{-1/2})\text{ \ and \ }%
T^{-1}\sum_{t\leq T}\eta _{t}(i,i^{\prime })=O_{p}(T^{-1/2}),
\label{P_I_L1_1}
\end{equation}%
where\ $\eta _{t}(i,i^{\prime })\equiv R_{i,t}R_{i^{\prime },t}-\mathrm{E}%
[R_{i,t}R_{i^{\prime },t}]$. Under Assumptions \ref{A1}(i, ii), we apply the
covariance inequality for strong mixing processes (see, e.g., Corollary 14.3
of \cite{davidsonbook}) to show that%
\begin{eqnarray}
\mathrm{E}\left[ \left( T^{-1/2}\sum_{t\leq T}(R_{i,t}-\mu _{i})\right) ^{2}%
\right] &=&T^{-1}\sum_{t\leq T}\mathrm{Var}(R_{i,t})+2T^{-1}\sum_{t=2}^{T}%
\sum_{s=1}^{t-1}\mathrm{Cov}(R_{i,t},R_{i,s})  \notag \\
&\leq &C+CT^{-1}\sum_{t=2}^{T}\sum_{s=1}^{t-1}\alpha _{t-s}^{1-4/r}\left
\Vert R_{i,t}\right \Vert _{r/2}\left \Vert R_{i,s}\right \Vert _{r/2} 
\notag \\
&\leq &C+CT^{-1}\sum_{j=1}^{T-1}(T-j)\alpha _{j}^{1-4/r}\leq C.
\label{P_I_L1_1b}
\end{eqnarray}%
Using Markov's inequality, the first part of (\ref{P_I_L1_1}) follows
directly. Next, under\ Assumption \ref{A1}(ii) and by H\"{o}lder's
inequality, we have:%
\begin{equation}
\mathrm{E}\left[ |\eta _{t}(i,i^{\prime })|^{r/2}\right] \leq C\mathrm{E}%
\left[ |R_{i,t}R_{i^{\prime },t}|^{r/2}\right] \leq C(\mathrm{E}\left[
|R_{i,t}|^{r}\right] \mathrm{E}\left[ |R_{i^{\prime },t}|^{r}\right]
)^{1/2}\leq C.  \label{P_I_L1_2}
\end{equation}%
Therefore, applying the covariance inequality for strong mixing processes
and using the bound in (\ref{P_I_L1_2}), we get%
\begin{eqnarray}
\mathrm{E}\left[ \left( T^{-1/2}\sum_{t\leq T}\eta _{t}(i,i^{\prime
})\right) ^{2}\right] &=&T^{-1}\sum_{t\leq T}\mathrm{Var}(\eta
_{t}(i,i^{\prime }))+2T^{-1}\sum_{t=2}^{T}\sum_{s=1}^{t-1}\mathrm{Cov}(\eta
_{t}(i,i^{\prime }),\eta _{s}(i,i^{\prime }))  \notag \\
&\leq &C+CT^{-1}\sum_{t=2}^{T}\sum_{s=1}^{t-1}\alpha _{t-s}^{1-4/r}\left
\Vert \eta _{t}(i,i^{\prime })\right \Vert _{r/2}\left \Vert \eta
_{s}(i,i^{\prime })\right \Vert _{r/2}  \notag \\
&\leq &C+CT^{-1}\sum_{j=1}^{T-1}(T-j)\alpha _{j}^{1-4/r}\leq C.
\label{P_I_L1_3}
\end{eqnarray}%
Thus, the second part of (\ref{P_I_L1_1}) follows from (\ref{P_I_L1_3}) and
Markov's inequality.

(ii) By the definition of $\tilde{R}_{-i,t}$, it is sufficient to show that\
for any $i,i^{\prime }\leq d$,%
\begin{equation}
T^{-1/2}\sum_{t\leq T}\varepsilon _{i,t}=O_{p}(1)\text{ \ and \ }%
T^{-1/2}\sum_{t\leq T}R_{i^{\prime },t}\varepsilon _{i,t}=O_{p}(1).
\label{P_I_L1_4}
\end{equation}%
In the proof of Theorem \ref{T2}, we have established that%
\begin{equation}
C^{-1}\leq \lambda _{\min }(Q)\leq \lambda _{\max }(Q)\leq C.
\label{P_I_L1_5}
\end{equation}%
Using Assumptions \ref{A1}(ii, iii) and (\ref{P_I_L1_5}), we obtain:%
\begin{eqnarray}
\max_{i\leq d}\left \Vert \beta _{i}\right \Vert ^{2} &=&\max_{i\leq d}%
\mathrm{Cov}(R_{-i},R_{i})^{\top }\mathrm{Var}(R_{-i})^{-2}\mathrm{Cov}%
(R_{-i},R_{i})  \notag \\
&\leq &\frac{\max_{i\leq d}\mathrm{Cov}(R_{-i},R_{i})^{\top }\mathrm{Var}%
(R_{-i})^{-1}\mathrm{Cov}(R_{-i},R_{i})}{\lambda _{\min }(Q)}  \notag \\
&\leq &C\max_{i\leq d}\mathrm{Var}(R_{i})\leq C.  \label{P_I_L1_6}
\end{eqnarray}%
Since $\varepsilon _{i,t}=(R_{i,t}-\mu _{i})-(R_{-i,t}-\mu _{-i})^{\top
}\beta _{i}$, in view of (\ref{P_I_L1_6}), we can apply the Cauchy-Schwarz
inequality to obtain: 
\begin{equation}
\left \vert \sum_{t\leq T}\varepsilon _{i,t}\right \vert ^{2}=\left \vert
\sum_{t\leq T}\left( (R_{i,t}-\mu _{i})-(R_{-i,t}-\mu _{-i})^{\top }\beta
_{i}\right) \right \vert ^{2}\leq C\sum_{i\leq d}\left \vert \sum_{t\leq
T}(R_{i,t}-\mu _{i})\right \vert ^{2}.  \label{P_I_L1_9}
\end{equation}%
Since we have shown that $T^{-1}\sum_{t\leq T}(R_{i,t}-\mu
_{i})=O_{p}(T^{-1/2})$ in (\ref{P_I_L1_1}), the first claim in (\ref%
{P_I_L1_4}) follows from (\ref{P_I_L1_9}). Similarly,\ for any $i^{\prime
}\neq i$, we have: 
\begin{eqnarray}
\left \vert \sum_{t\leq T}R_{i^{\prime },t}\varepsilon _{i,t}\right \vert
^{2} &=&\left \vert \sum_{t\leq T}\left( R_{i^{\prime },t}\varepsilon _{i,t}-%
\mathrm{E}\left[ R_{i^{\prime },t}\varepsilon _{i,t}\right] \right) \right
\vert ^{2}  \notag \\
&\leq &C\sum_{i\leq d}\left( \left \vert \sum_{t\leq T}\eta _{t}(i^{\prime
},i)\right \vert +\left \vert \mu _{i}-\mu _{-i}^{\top }\beta _{i}\right
\vert \left \vert \sum_{t\leq T}(R_{i^{\prime },t}-\mu _{i^{\prime }})\right
\vert \right) .  \label{P_I_L1_10}
\end{eqnarray}%
Since $\max_{i\leq d}\left \vert \mu _{i}-\mu _{-i}^{\top }\beta _{i}\right
\vert \leq C$ by Assumption \ref{A1}(ii) and (\ref{P_I_L1_6}), the second
claim in (\ref{P_I_L1_4}) holds by (\ref{P_I_L1_1}) and (\ref{P_I_L1_10}).

(iii) By the definition of the LS estimator, 
\begin{equation}
(\hat{\alpha}_{i}-\alpha _{i},\hat{\beta}_{i}^{\top }-\beta _{i}^{\top
})^{\top }=\hat{Q}_{-i}T^{-1}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t}.  \label{P_I_L1_11}
\end{equation}%
From part (i) of the lemma and the inequalities in (\ref{P_I_L1_5}), we have
wpa1:%
\begin{equation}
C^{-1}\leq \lambda _{\min }(\hat{Q})\leq \lambda _{\max }(\hat{Q})\leq C.
\label{P_I_L1_12a}
\end{equation}%
Since\ $\hat{Q}_{-i}$ for $i=1,\ldots ,d$ are submatrices of $\hat{Q}$, it
follows that 
\begin{equation}
C^{-1}\leq \min_{i\leq d}\lambda _{\min }(\hat{Q}_{-i})\leq \max_{i\leq
d}\lambda _{\max }(\hat{Q}_{-i})\leq C,  \label{P_I_L1_12}
\end{equation}%
wpa1. Therefore,\ we can write:%
\begin{eqnarray*}
\max_{i\leq d}(\left \vert \hat{\alpha}_{i}-\alpha _{i}\right \vert ^{2}+||%
\hat{\beta}_{i}-\beta _{i}||^{2}) &=&\max_{i\leq d}\left( T^{-1}\sum_{t\leq
T}\tilde{R}_{-i,t}\varepsilon _{i,t}\right) ^{\top }\hat{Q}_{-i}^{2}\left(
T^{-1}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}\right) \\
&\leq &\frac{\max_{i\leq d}\left \Vert T^{-1}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}\right \Vert ^{2}}{\lambda _{\min }(\hat{Q}_{-i})}%
=O_{p}(T^{-1}),
\end{eqnarray*}%
where the last equality follows from (\ref{P_I_L1_12}) and part (ii) of the
lemma.\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{I_L2}\ Under Assumption \ref{A1}, we have:%
\begin{equation*}
\max_{i\leq d}\max_{j=1,2}\left \vert \frac{T^{1/2}(\hat{\theta}%
_{i,j}-\theta _{i,j})}{\hat{s}_{i,j}}-\frac{A_{j,\cdot
}Q_{-i}^{-1}T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}}{s_{i,j}%
}\right \vert =O_{p}(T^{-1/2}).
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.}\ Starting from the expression for $T^{1/2}(\hat{%
\theta}_{i}-\theta _{i})$ in\ (\ref{OLS_Exp}), we have%
\begin{eqnarray}
&&\frac{T^{1/2}(\hat{\theta}_{i,j}-\theta _{i,j})}{\hat{s}_{i,j}}-\frac{%
A_{j,\cdot }Q_{-i}^{-1}T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t}}{s_{i,j}}  \notag \\
&=&(\hat{s}_{i,j}^{-1}-s_{i,j}^{-1})A_{j,\cdot }\hat{Q}_{-i}^{-1}T^{-1/2}%
\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}+\frac{A_{j,\cdot }(\hat{Q}%
_{-i}^{-1}-Q_{-i}^{-1})T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t}}{s_{i,j}}.  \label{P_I_L2_1}
\end{eqnarray}%
By the Cauchy-Schwarz inequality, we can bound the first term on the
right-hand side of the above equation as follows:%
\begin{eqnarray}
&&\max_{i\leq d}\max_{j=1,2}\left \vert (\hat{s}%
_{i,j}^{-1}-s_{i,j}^{-1})A_{j,\cdot }\hat{Q}_{-i}^{-1}T^{-1/2}\sum_{t\leq T}%
\tilde{R}_{-i,t}\varepsilon _{i,t}\right \vert  \notag \\
&\leq &\max_{i\leq d}\max_{j=1,2}\frac{s_{i,j}^{2}}{\hat{s}_{i,j}(\hat{s}%
_{i,j}+s_{i,j})}\left \Vert \frac{A_{j,\cdot }\hat{Q}_{-i}^{-1}T^{-1/2}%
\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}}{s_{i,j}}\right \Vert \left
\vert \frac{\hat{s}_{i,j}^{2}}{s_{i,j}^{2}}-1\right \vert  \notag \\
&\leq &C\max_{i\leq d}\left \Vert T^{-1/2}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}\right \Vert \max_{i\leq d}\max_{j=1,2}\left \vert 
\frac{\hat{s}_{i,j}^{2}}{s_{i,j}^{2}}-1\right \vert ,  \label{P_I_L2_2}
\end{eqnarray}%
wpa1, where the second inequality follows from (\ref{P_I_L1_18}), (\ref%
{P_I_L1_5}), (\ref{P_I_L1_12}), and Lemma \ref{I_L1b}.\ Thus, by (\ref%
{P_I_L2_2}), we can invoke Lemma \ref{I_L1b} and Lemma \ref{I_L1}(ii) to
conclude:%
\begin{equation}
\max_{i\leq d}\max_{j=1,2}\left \vert A_{j,\cdot }\hat{Q}_{-i}^{-1}\left(
T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}\right) \left( \frac{%
1}{\hat{s}_{i,j}}-\frac{1}{s_{i,j}}\right) \right \vert =O_{p}(T^{-1/2}).
\label{P_I_L2_3}
\end{equation}%
Next, by Lemma \ref{I_L1}(i, ii), (\ref{P_I_L1_18}), (\ref{P_I_L1_5}) and (%
\ref{P_I_L1_12}),\ we can bound the second term on the right-hand side of (%
\ref{P_I_L2_1}):%
\begin{eqnarray}
&&\max_{i\leq d}\max_{j=1,2}\left \vert \frac{A_{j,\cdot }(\hat{Q}%
_{-i}^{-1}-Q_{-i}^{-1})\left( T^{-1/2}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}\right) }{s_{i,j}}\right \vert  \notag \\
&\leq &\max_{i\leq d}\max_{j=1,2}\frac{(\lambda _{\max }(Q))^{1/2}}{\sigma
_{\varepsilon _{i}}}\left \Vert \hat{Q}_{-i}^{-1}-Q_{-i}^{-1}\right \Vert
\left \Vert T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}\right
\Vert =O_{p}(T^{-1/2}).  \label{P_I_L2_4}
\end{eqnarray}%
The claim of the lemma then follows from\ (\ref{P_I_L2_1}), (\ref{P_I_L2_3})
and (\ref{P_I_L2_4}).\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L1_a}\ For any generic function\ $g(\cdot )$\ of $R_{t}$,\ we have:%
\begin{eqnarray*}
\mathrm{E}^{\ast }\left[ (m\ell )^{-1}\sum_{t\leq m\ell }g(\tilde{R}_{t}^{b})%
\right] &=&\ell ^{-1}\mathrm{E}^{\ast }\left[ \sum_{l\leq \ell }g(\tilde{R}%
_{l}^{b})\right] \\
&=&q^{-1}\sum_{t\leq T}g(\tilde{R}_{t})-q^{-1}\sum_{t\leq \ell -1}(1-t/\ell
)(g(\tilde{R}_{t})+g(\tilde{R}_{T-t+1})).
\end{eqnarray*}
\end{lemma}

\noindent \textsc{Proof.} We begin the proof by writing: 
\begin{equation*}
(m\ell )^{-1}\sum_{t\leq m\ell }g(\tilde{R}_{t}^{b})=(m\ell
)^{-1}\sum_{j\leq m}\sum_{l\leq \ell }g(\tilde{R}_{\ell (j-1)+l}^{b}).
\end{equation*}%
Since $\sum_{l\leq \ell }g(\tilde{R}_{\ell (j-1)+l}^{b})$ only depends on $%
Z_{j}^{b}\equiv (\tilde{R}_{(j-1)\ell +1}^{b},\ldots ,\tilde{R}_{j\ell
}^{b}) $, which is i.i.d. across $j$ given the data, we deduce that%
\begin{equation}
\mathrm{E}^{\ast }\left[ \sum_{t\leq m\ell }g(\tilde{R}_{t}^{b})\right]
=\sum_{j\leq m}\mathrm{E}^{\ast }\left[ \sum_{l\leq \ell }g(\tilde{R}_{\ell
(j-1)+l}^{b})\right] =m\mathrm{E}^{\ast }\left[ \sum_{l\leq \ell }g(\tilde{R}%
_{l}^{b})\right] .  \label{P_B_L1a_1}
\end{equation}%
Additionally,%
\begin{eqnarray*}
\mathrm{E}^{\ast }\left[ \sum_{l\leq \ell }g(\tilde{R}_{l}^{b})\right]
&=&q^{-1}\sum_{j^{\prime }\leq q}\sum_{l\leq \ell }g(\tilde{R}_{j^{\prime
}+l-1}) \\
&=&q^{-1}\left( \sum_{t\leq \ell -1}tg(\tilde{R}_{t})+\ell \sum_{\ell \leq
t\leq T-\ell +1}g(\tilde{R}_{t})+\sum_{T-\ell +2\leq t\leq T}(T-t+1)g(\tilde{%
R}_{t})\right) \\
&=&q^{-1}\left( \sum_{t\leq \ell -1}tg(\tilde{R}_{t})+\ell \sum_{\ell \leq
t\leq T-\ell +1}g(\tilde{R}_{t})+\sum_{t\leq \ell -1}tg(\tilde{R}%
_{T-t+1})\right) \\
&=&q^{-1}\left( \ell \sum_{t\leq T}g(\tilde{R}_{t})-\sum_{t\leq \ell
-1}(\ell -t)(g(\tilde{R}_{t})+g(\tilde{R}_{T-t+1}))\right) ,
\end{eqnarray*}%
which, along with (\ref{P_B_L1a_1}) shows the claim of the lemma.\hfill $%
Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L1_b}\ For any generic functions\ $g_{1}(\cdot )$\ and $g_{2}(\cdot
)$\ of $R_{t}$, let $G_{t_{1},t_{2}}=g_{1}(\tilde{R}_{t_{1}})g_{2}(\tilde{R}%
_{t_{2}})$. Then we have:%
\begin{equation*}
\mathrm{E}^{\ast }\left[ \ell ^{-1}\sum_{l,l^{\prime }\leq \ell }g_{1}(%
\tilde{R}_{l}^{b})g_{2}(\tilde{R}_{l^{\prime }}^{b})\right] =q^{-1}\left(
\sum_{t\leq T}G_{t,t}+\sum_{1\leq h\leq \ell -1}\left( 1-\frac{h}{\ell }%
\right) \sum_{t\leq T-h}\left( G_{t,t+h}+G_{t+h,t}\right) \right) -C_{T},
\end{equation*}%
where%
\begin{eqnarray*}
C_{T} &\equiv &\sum_{t=1}^{\ell -1}\frac{\ell -t}{q\ell }%
(G_{t,t}+G_{T+1-t,T+1-t}) \\
&&+\sum_{h=1}^{\ell -1}\sum_{t=1}^{\ell -h-1}\frac{\ell -t-h}{q\ell }%
(G_{t,t+h}+G_{t+h,t}+G_{T-h+1-t,T+1-t}+G_{T+1-t,T-h+1-t}).
\end{eqnarray*}
\end{lemma}

\noindent \textsc{Proof.} By the property of $Z_{j}^{b}\equiv (\tilde{R}%
_{(j-1)\ell +1}^{b},\ldots ,\tilde{R}_{j\ell }^{b})$,\ we obtain:%
\begin{equation}
\mathrm{E}^{\ast }\left[ \ell ^{-1}\sum_{l,l^{\prime }\leq \ell }g_{1}(%
\tilde{R}_{l}^{b})g_{2}(\tilde{R}_{l^{\prime }}^{b})\right] =(q\ell
)^{-1}\sum_{j\leq q}\left( \sum_{l,l^{\prime }\leq \ell }g_{1}(\tilde{R}%
_{j+l-1})g_{2}(\tilde{R}_{j+l^{\prime }-1})\right) .  \label{P_B_L1b_1}
\end{equation}%
Let $(u_{i,i^{\prime }})_{i,i^{\prime }\leq T}$ denote a matrix where%
\begin{equation*}
(u_{i,i^{\prime }})_{j\leq i,i^{\prime }\leq j+\ell -1}=(g_{1}(\tilde{R}%
_{j+l-1})g_{2}(\tilde{R}_{j+l^{\prime }-1}))_{l,l^{\prime }\leq \ell }\text{
\ for any }j\leq q,
\end{equation*}%
with all other elements of\ $(u_{i,i^{\prime }})_{i,i^{\prime }\leq T}$ are\
zero. Then $\sum_{j\leq q}\sum_{l,l^{\prime }\leq \ell }g_{1}(\tilde{R}%
_{j+l-1})g_{2}(\tilde{R}_{j+l^{\prime }-1})$ equals the sum of the entries
of $(u_{i,i^{\prime }})_{i,i^{\prime }\leq T}$ with the following
contributions. For the elements on the diagonal of $(u_{i,i^{\prime
}})_{i,i^{\prime }\leq T}$: (i) entries from the $\ell $-th row to the $%
(T-\ell +1)$-th row added $\ell $ times; (ii) entries in the $i$-th row for $%
i\leq \ell -1$ added $i$ times; and (iii) entries in the $i^{\prime }$-th
row for $i^{\prime }\geq T-\ell +2$ added $T-i^{\prime }+1$ times. For the $%
h $-th ($h=1,\ldots ,\ell -1$) off-diagonal elements of $(u_{i,i^{\prime
}})_{i,i^{\prime }\leq T}$: (i) entries from the $(\ell -h)$-th row to the $%
(T-\ell +1)$-th row added $\ell -h$ times; (ii) entries in the $i$-th row
for $i\leq \ell -h-1$ added $i$ times; and (iii) entries in the $i^{\prime }$%
-th row for $T-\ell +2\leq i^{\prime }\leq T-h$ added $T-h-i^{\prime }+1$
times. Under this structure, it is clear that contribution of the diagonal
entries of $(u_{i,i^{\prime }})_{i,i^{\prime }\leq T}$, denoted as\ $C_{u,0}$%
, to $\sum_{j\leq q}\sum_{l,l^{\prime }\leq \ell }g_{1}(\tilde{R}%
_{j+l-1})g_{2}(\tilde{R}_{j+l^{\prime }-1})$ is:%
\begin{eqnarray}
C_{u,0} &=&\sum_{t\leq \ell -1}tG_{t,t}+\ell \sum_{\ell \leq t\leq T-\ell
+1}G_{t,t}+\sum_{T-\ell +2\leq t\leq T}(T-t+1)G_{t,t}  \notag \\
&=&\ell \sum_{t\leq T}G_{t,t}-\sum_{t\leq \ell -1}(\ell
-t)(G_{t,t}+G_{T+1-t,T+1-t}).  \label{P_B_L1b_2}
\end{eqnarray}%
Similarly, the contribution from the $h$-th ($h=1,\ldots ,\ell -1$) upper
off-diagonal of $(u_{i,i^{\prime }})_{i,i^{\prime }\leq T}$,\ denoted as $%
C_{u,h}$, satisfies:%
\begin{eqnarray}
C_{u,h} &=&\sum_{t\leq \ell -h-1}tG_{t,t+h}+(\ell -h)\sum_{\ell -h\leq t\leq
T-\ell +1}G_{t,t+h}+\sum_{T-\ell +2\leq t\leq T-h}(T-t+1-h)G_{t,t+h}  \notag
\\
&=&(\ell -h)\sum_{1\leq t\leq T-h}G_{t,t+h}-\sum_{t\leq \ell -h-1}(\ell
-t-h)(G_{t,t+h}+G_{T-h+1-t,T+1-t}),  \label{P_B_L1b_3}
\end{eqnarray}%
and the contribution from the $h$-th ($h=1,\ldots ,\ell -1$) lower
off-diagonal of $(u_{i,i^{\prime }})_{i,i^{\prime }\leq T}$,\ denoted as $%
C_{u,-h}$, satisfies:%
\begin{equation}
C_{u,-h}=(\ell -h)\sum_{1\leq t\leq T-h}G_{t+h,t}-\sum_{t\leq \ell
-h-1}(\ell -t-h)(G_{t+h,t}+G_{T+1-t,T-h+1-t}).  \label{P_B_L1b_4}
\end{equation}%
Since the remaining elements in $(u_{i,i^{\prime }})_{i,i^{\prime }\leq T}$
which are not accounted for in $C_{u,0}$, $C_{u,h}$ and\ $C_{u,-h}$ are
zero, we deduce that 
\begin{equation*}
\sum_{j\leq q}\sum_{l,l^{\prime }\leq \ell }g_{1}(\tilde{R}_{j+l-1})g_{2}(%
\tilde{R}_{j+l^{\prime }-1})=C_{u,0}+\sum_{1\leq h\leq \ell
-1}(C_{u,h}+C_{u,-h}),
\end{equation*}%
which, along with (\ref{P_B_L1b_2}), (\ref{P_B_L1b_3}) and (\ref{P_B_L1b_4}%
), shows the claim of the lemma.\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L1_c}\ Under Assumption \ref{A1}, for any $i\leq d$ we have:%
\begin{equation*}
(m\ell )^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }[\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}]=T^{-1}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}+O_{p}(\ell ^{1/2}T^{-1})=O_{p}(T^{-1/2}).
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} Applying Lemma \ref{B_L1_a}, we can write:%
\begin{eqnarray}
&&\mathrm{E}^{\ast }\left[ (m\ell )^{-1}\sum_{t\leq m\ell }\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}\right] -T^{-1}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}  \notag \\
&=&(Tq^{-1}-1)T^{-1}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t}-q^{-1}\sum_{t\leq \ell -1}\left( 1-t/\ell \right) (\tilde{R}%
_{-i,t}\varepsilon _{i,t}+\tilde{R}_{-i,T-t+1}\varepsilon _{i,T-t+1}).
\label{P_B_L1c_1}
\end{eqnarray}%
Since\ $Tq^{-1}-1=O(\ell T^{-1})$, by Lemma \ref{I_L1}(ii), we have 
\begin{equation}
(Tq^{-1}-1)T^{-1}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}=O_{p}(\ell
T^{-3/2}).  \label{P_B_L1c_2}
\end{equation}%
Similarly, we can show that 
\begin{equation}
q^{-1}\sum_{t\leq \ell -1}(1-t/\ell )(\tilde{R}_{-i,t}\varepsilon _{i,t}+%
\tilde{R}_{-i,T-t+1}\varepsilon _{i,T-t+1})=O_{p}(\ell ^{1/2}T^{-1}),
\label{P_B_L1c_3}
\end{equation}%
which, together with Lemma \ref{I_L1}(ii), (\ref{P_B_L1c_1}) and (\ref%
{P_B_L1c_2}), establishes the claim of the lemma.\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L1_d}\ Under Assumptions \ref{A1} and \ref{A2},\ we have:%
\begin{eqnarray*}
&&\mathrm{Cov}^{\ast }\left( (m\ell )^{-1/2}\sum_{t\leq m\ell }\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b},(m\ell )^{-1/2}\sum_{t\leq m\ell }\tilde{R}%
_{-i^{\prime },t}^{b}\varepsilon _{i^{\prime },t}^{b}\right) \\
\text{ \  \ } &=&\mathrm{Cov}\left( T^{-1/2}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t},T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i^{\prime
},t}\varepsilon _{i^{\prime },t}\right) +O_{p}(\ell ^{2}T^{-1+2/\tilde{r}%
}+\ell ^{-1}),
\end{eqnarray*}%
for any $i,i^{\prime }\leq d$.
\end{lemma}

\noindent \textsc{Proof.} Since $Z_{j}^{b}\equiv (\tilde{R}_{(j-1)\ell
+1}^{b},\ldots ,\tilde{R}_{j\ell }^{b})$ are i.i.d. across $j$ given the
data,%
\begin{eqnarray}
&&\mathrm{Cov}^{\ast }\left( \sum_{t\leq m\ell }\tilde{R}_{-i,t}^{b}%
\varepsilon _{i,t}^{b},\sum_{t\leq m\ell }\tilde{R}_{-i^{\prime
},t}^{b}\varepsilon _{i^{\prime },t}^{b}\right)  \notag \\
&=&\mathrm{Cov}^{\ast }\left( \sum_{j\leq m}\sum_{l\leq \ell }\tilde{R}%
_{-i,\ell (j-1)+l}^{b}\varepsilon _{i,\ell (j-1)+l}^{b},\sum_{j\leq
m}\sum_{l\leq \ell }\tilde{R}_{-i^{\prime },\ell (j-1)+l}^{b}\varepsilon
_{i^{\prime },\ell (j-1)+l}^{b}\right)  \notag \\
&=&m\mathrm{Cov}^{\ast }\left( \sum_{l\leq \ell }\tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b},\sum_{l\leq \ell }\tilde{R}_{-i^{\prime
},l}^{b}\varepsilon _{i^{\prime },l}^{b}\right) ,  \label{P_B_L1_d_0}
\end{eqnarray}%
where%
\begin{eqnarray}
\mathrm{Cov}^{\ast }\left( \sum_{l\leq \ell }\tilde{R}_{-i,l}^{b}\varepsilon
_{i,l}^{b},\sum_{l\leq \ell }\tilde{R}_{-i^{\prime },l}^{b}\varepsilon
_{i^{\prime },l}^{b}\right) &=&\mathrm{E}^{\ast }\left[ \left( \sum_{l\leq
\ell }\tilde{R}_{-i,l}^{b}\varepsilon _{i,l}^{b}\right) \sum_{l\leq \ell }(%
\tilde{R}_{-i^{\prime },l}^{b}\varepsilon _{i^{\prime },l}^{b})^{\top }%
\right]  \notag \\
&&-\left( \sum_{l\leq \ell }\mathrm{E}^{\ast }[\tilde{R}_{-i,l}^{b}%
\varepsilon _{i,l}^{b}]\right) \sum_{l\leq \ell }\mathrm{E}^{\ast }[(\tilde{R%
}_{-i^{\prime },l}^{b}\varepsilon _{i^{\prime },l}^{b})^{\top }].
\label{P_B_L1_d_1}
\end{eqnarray}%
By Lemma \ref{B_L1_c}, we have for any $i\leq d$: 
\begin{equation*}
\ell ^{-1}\sum_{l\leq \ell }\mathrm{E}^{\ast }[\tilde{R}_{-i,l}^{b}%
\varepsilon _{i,l}^{b}]=(m\ell )^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }[%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}]=O_{p}(T^{-1/2}),
\end{equation*}%
which, along with (\ref{P_B_L1_d_0}) and (\ref{P_B_L1_d_1}), shows that%
\begin{eqnarray}
&&\mathrm{Cov}^{\ast }\left( (m\ell )^{-1/2}\sum_{t\leq m\ell }\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b},(m\ell )^{-1/2}\sum_{t\leq m\ell }\tilde{R}%
_{-i^{\prime },t}^{b}\varepsilon _{i^{\prime },t}^{b}\right)  \notag \\
&=&\ell ^{-1}\mathrm{E}^{\ast }\left[ \left( \sum_{l\leq \ell }\tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b}\right) \sum_{l\leq \ell }(\tilde{R}%
_{-i^{\prime },l}^{b}\varepsilon _{i^{\prime },l}^{b})^{\top }\right]
+O_{p}(\ell T^{-1}).  \label{P_B_L1_d_2}
\end{eqnarray}

Let $\nu _{1,t,h}\equiv \tilde{R}_{-i,t}\tilde{R}_{-i^{\prime },t+h}^{\top
}\varepsilon _{i,t}\varepsilon _{i^{\prime },t+h}$ and $\nu _{2,t,h}\equiv 
\tilde{R}_{-i,T+1-t}\tilde{R}_{-i^{\prime },T+1-t-h}^{\top }\varepsilon
_{i,T+1-t}\varepsilon _{i^{\prime },T+1-t-h}$. Applying Lemma \ref{B_L1_b}
componentwisely to the first term in the right-hand side of (\ref{P_B_L1_d_2}%
), we obtain:%
\begin{eqnarray}
&&\ell ^{-1}\mathrm{E}^{\ast }\left[ \left( \sum_{l\leq \ell }\tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b}\right) \sum_{l\leq \ell }(\tilde{R}%
_{-i^{\prime },l}^{b}\varepsilon _{i^{\prime },l}^{b})^{\top }\right]  \notag
\\
&=&q^{-1}\left( \sum_{t\leq T}\nu _{1,t,0}+\sum_{1\leq h\leq \ell -1}\left(
1-\frac{h}{\ell }\right) \sum_{t\leq T-h}\left( \nu _{1,t,h}+\nu
_{1,t+h,-h}\right) \right) -C_{R,T},  \label{P_B_L1_d_3}
\end{eqnarray}%
where%
\begin{eqnarray}
C_{R,T} &\equiv &\sum_{t=1}^{\ell -1}\frac{\ell -t}{q\ell }(\nu _{1,t,0}+\nu
_{1,T+1-t,0})  \notag \\
&&+\sum_{h=1}^{\ell -1}\sum_{t=1}^{\ell -h-1}\frac{\ell ^{2}-t-h}{q\ell }%
(\nu _{1,t,h}+\nu _{1,t+h,-h}+\nu _{2,t,h}+\nu _{2,t+h,-h}).
\label{P_B_L1_d_4}
\end{eqnarray}

By the covariance inequality for strong mixing processes, for any $%
i_{1},i_{2},i_{1}^{\prime },i_{2}^{\prime }\leq i$ with $i_{1}\neq
i_{1}^{\prime }$\ and $i_{2}\neq i_{2}^{\prime }$,\ we have%
\begin{equation}
\mathrm{E}\left[ |R_{i_{1},t}R_{i_{2},t+h}\varepsilon _{i_{1}^{\prime
},t}\varepsilon _{i_{2}^{\prime },t+h}|\right] \leq C\alpha
_{h}^{1-4/r}\left \Vert R_{i_{1},t}\varepsilon _{i_{1}^{\prime },t}\right
\Vert _{r/2}\left \Vert R_{i_{2},t+h}\varepsilon _{i_{2}^{\prime
},t+h}\right \Vert _{r/2}\leq C\alpha _{h}^{1-4/r},  \label{P_B_L1_d_5a}
\end{equation}%
where the second inequality is by (\ref{P_I_L3_4}). Similarly, we can show
that%
\begin{equation}
\mathrm{E}\left[ |R_{i_{1},t}\varepsilon _{i_{1}^{\prime },t}\varepsilon
_{i_{2}^{\prime },t+h}|+|R_{i_{2},t+h}\varepsilon _{i_{1}^{\prime
},t}\varepsilon _{i_{2}^{\prime },t+h}|+|\varepsilon _{i_{1}^{\prime
},t}\varepsilon _{i_{2}^{\prime },t+h}|\right] \leq C\alpha _{h}^{1-4/r}.
\label{P_B_L1_d_5b}
\end{equation}%
From (\ref{P_B_L1_d_5a}) and (\ref{P_B_L1_d_5b}), it follows that%
\begin{equation}
\mathrm{E}\left[ ||\nu _{1,t,h}||+||\nu _{2,t,h}||\right] \leq C\alpha
_{h}^{1-4/r}.  \label{P_B_L1_d_6}
\end{equation}%
Therefore, by the triangle inequality and (\ref{P_B_L1_d_6}),%
\begin{eqnarray*}
\mathrm{E}\left[ \left \Vert C_{R,T}\right \Vert \right] &\leq
&\sum_{t=1}^{\ell -1}\frac{\ell -t}{q\ell }\mathrm{E}\left[ ||\nu
_{1,t,0}||+||\nu _{1,T+1-t,0}||\right] \\
&&+\sum_{h=1}^{\ell -1}\sum_{t=1}^{\ell -h-1}\frac{\ell -t-h}{q\ell }\mathrm{%
E}\left[ ||\nu _{1,t,h}||+||\nu _{1,t+h,-h}||+||\nu _{2,t,h}||+||\nu
_{2,t+h,-h}||\right] \\
&\leq &Cq^{-1}\sum_{h=0}^{\ell -1}\sum_{t=1}^{\ell -h-1}\alpha
_{h}^{1-4/r}\leq C\ell q^{-1}\sum_{h=0}^{\ell -1}\alpha _{h}^{1-4/r}\leq
C\ell T^{-1},
\end{eqnarray*}%
which together with Markov's inequality implies that 
\begin{equation}
C_{R,T}=O_{p}(\ell T^{-1}).  \label{P_B_L1_d_7}
\end{equation}%
Collecting the results in (\ref{P_B_L1_d_2}), (\ref{P_B_L1_d_3}) and (\ref%
{P_B_L1_d_7}), we obtain%
\begin{eqnarray*}
&&\mathrm{Cov}^{\ast }\left( (m\ell )^{-1/2}\sum_{t\leq m\ell }\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b},(m\ell )^{-1/2}\sum_{t\leq m\ell }\tilde{R}%
_{-i^{\prime },t}^{b}\varepsilon _{i^{\prime },t}^{b}\right) \\
&=&q^{-1}\left( \sum_{t\leq T}\nu _{1,t,0}+\sum_{1\leq h\leq \ell -1}\frac{%
\ell -h}{\ell }\sum_{t\leq T-h}\left( \nu _{1,t,h}+\nu _{1,t+h,-h}\right)
\right) +O_{p}(\ell T^{-1}).
\end{eqnarray*}%
Therefore, the claim of the lemma follows if%
\begin{eqnarray}
&&q^{-1}\left( \sum_{t\leq T}\nu _{1,t,0}+\sum_{1\leq h\leq \ell -1}\frac{%
\ell -h}{\ell }\sum_{t\leq T-h}\left( \nu _{1,t,h}+\nu _{1,t+h,-h}\right)
\right)  \notag \\
&=&\mathrm{Cov}\left( T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t},T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i^{\prime },t}\varepsilon
_{i^{\prime },t}\right) +O_{p}(\ell ^{2}T^{-1+2/\tilde{r}}+\ell ^{-1}).
\label{P_B_L1_d_8}
\end{eqnarray}

For $k,k^{\prime }\leq d$, let $\nu _{1,t,h}(k,k^{\prime })$ denote the
entry of $\nu _{1,t,h}$ on its $k$-th row and $k^{\prime }$-th column. By
the triangle inequality%
\begin{eqnarray}
&&\left \Vert q^{-1}\sum_{h=0}^{\ell -1}\frac{\ell -h}{\ell }\sum_{t\leq
T-h}\left( \nu _{1,t,h}(k,k^{\prime })-\mathrm{E}\left[ \nu
_{1,t,h}(k,k^{\prime })\right] \right) \right \Vert _{\tilde{r}/4}  \notag \\
&\leq &q^{-1}\sum_{h=0}^{\ell -1}\left \Vert \sum_{t\leq T-h}\left( \nu
_{1,t,h}(k,k^{\prime })-\mathrm{E}\left[ \nu _{1,t,h}(k,k^{\prime })\right]
\right) \right \Vert _{\tilde{r}/4}.  \label{P_B_L1_d_9}
\end{eqnarray}%
Let $\mathcal{F}_{t}$ denote the sigma algebra generated by $\left \{
R_{s}\right \} _{1\leq s\leq t}$. Applying the inequality in (1) in \cite%
{de2000strong} with $\beta =\tilde{r}/4$ and $\gamma =r/4$\ leads to%
\begin{eqnarray}
&&\left \Vert \mathrm{E}\left[ \nu _{1,t,h}(k,k^{\prime })|\mathcal{F}%
_{t+h-m}\right] -\mathrm{E}\left[ \nu _{1,t,h}(k,k^{\prime })\right] \right
\Vert _{\tilde{r}/4}  \notag \\
&\leq &\left( 12\alpha _{m-h}^{4/\tilde{r}-4/r}I\{m>h\}+2I\{m\leq h\}
\right) \left \Vert \tilde{R}_{-i,t}\varepsilon _{i,t}\right \Vert
_{r/2}\left \Vert \tilde{R}_{-i^{\prime },t+h}\varepsilon _{i^{\prime
},t+h}\right \Vert _{r/2}.  \label{P_B_L1_d_10}
\end{eqnarray}%
Following similar arguments in the proof of Theorem 3 in \cite{de2000strong}%
, we can use Lemma 2 in \cite{hansen1991strong} to obtain%
\begin{eqnarray*}
&&\left \Vert \sum_{t\leq T-h}\left( \nu _{1,t,h}(k,k^{\prime })-\mathrm{E}%
\left[ \nu _{1,t,h}(k,k^{\prime })\right] \right) \right \Vert _{\tilde{r}/4}
\\
&\leq &C\left( 1+2h\right) \left( \sum_{t\leq T-h}\left \Vert \tilde{R}%
_{-i,t}\varepsilon _{i,t}\right \Vert _{r/2}^{\tilde{r}/2}\left \Vert \tilde{%
R}_{-i^{\prime },t+h}\varepsilon _{i^{\prime },t+h}\right \Vert _{r/2}^{%
\tilde{r}/2}\right) ^{2/\tilde{r}}\leq CT^{2/\tilde{r}}(1+2h),
\end{eqnarray*}%
where the second inequality is by (\ref{P_I_L3_5}). This together with (\ref%
{P_B_L1_d_9}) shows that 
\begin{equation}
\left \Vert q^{-1}\sum_{h=0}^{\ell -1}\frac{\ell -h}{\ell }\sum_{t\leq
T-h}\left( \nu _{1,t,h}(k,k^{\prime })-\mathrm{E}\left[ \nu
_{1,t,h}(k,k^{\prime })\right] \right) \right \Vert _{\tilde{r}/4}\leq C\ell
^{2}T^{-1+2/\tilde{r}}.  \label{P_B_L1_d_11}
\end{equation}%
Similarly, we can show that 
\begin{equation}
\left \Vert q^{-1}\sum_{h=1}^{\ell -1}\frac{\ell -h}{\ell }\sum_{t\leq
T-h}\left( \nu _{1,t+h,-h}(k,k^{\prime })-\mathrm{E}\left[ \nu
_{1,t+h,-h}(k,k^{\prime })\right] \right) \right \Vert _{\tilde{r}/4}\leq
C\ell ^{2}T^{-1+2/\tilde{r}}.  \label{P_B_L1_d_11b}
\end{equation}%
Thus,\ by (\ref{P_B_L1_d_11}), (\ref{P_B_L1_d_11b})\ and Markov's inequality,%
\begin{eqnarray}
&&q^{-1}\left( \sum_{t\leq T}\nu _{1,t,0}+\sum_{h=1}^{\ell -1}\frac{\ell -h}{%
\ell }\sum_{t\leq T-h}\left( \nu _{1,t,h}+\nu _{1,t+h,-h}\right) \right) 
\notag \\
&=&q^{-1}\left( \sum_{t\leq T}\mathrm{E}\left[ \nu _{1,t,0}\right]
+\sum_{h=1}^{\ell -1}\frac{\ell -h}{\ell }\sum_{t\leq T-h}\left( \mathrm{E}%
\left[ \nu _{1,t,h}\right] +\mathrm{E}\left[ \nu _{1,t+h,-h}\right] \right)
\right) +O_{p}(\ell ^{2}T^{-1+2/\tilde{r}})  \notag \\
&=&\frac{T\mathrm{E}\left[ \nu _{1,1,0}\right] }{q}+\sum_{h=1}^{\ell -1}%
\frac{(\ell -h)(T-h)}{\ell q}\left( \mathrm{E}\left[ \nu _{1,1,h}\right] +%
\mathrm{E}\left[ \nu _{1,1+h,-h}\right] \right) +O_{p}(\ell ^{2}T^{-1+2/%
\tilde{r}}),  \label{P_B_L1_d_12}
\end{eqnarray}%
where the second equality follows from the stationarity of $R_{t}$. Next, we
observe that%
\begin{eqnarray}
&&\mathrm{Cov}\left( T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t},T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i^{\prime },t}\varepsilon
_{i^{\prime },t}\right)  \notag \\
&=&\mathrm{E}\left[ \nu _{1,1,0}\right] +\sum_{h=1}^{T-1}\frac{T-h}{T}\left( 
\mathrm{E}\left[ \nu _{1,1,h}\right] +\mathrm{E}\left[ \nu _{1,1+h,-h}\right]
\right) .  \label{P_B_L1_d_12b}
\end{eqnarray}%
Therefore,%
\begin{eqnarray}
&&\mathrm{Cov}\left( T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t},T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i^{\prime },t}\varepsilon
_{i^{\prime },t}\right)  \notag \\
&&-Tq^{-1}\left( \mathrm{E}\left[ \nu _{1,1,0}\right] +\sum_{h=1}^{\ell -1}%
\frac{(\ell -h)(T-h)}{\ell T}\left( \mathrm{E}\left[ \nu _{1,1,h}\right] +%
\mathrm{E}\left[ \nu _{1,1+h,-h}\right] \right) \right)  \notag \\
&=&(1-Tq^{-1})\mathrm{E}\left[ \nu _{1,1,0}\right] +\sum_{h=\ell
}^{T-1}(1-hT^{-1})\left( \mathrm{E}\left[ \nu _{1,1,h}\right] +\mathrm{E}%
\left[ \nu _{1,1+h,-h}\right] \right)  \notag \\
&&+\sum_{h=1}^{\ell -1}(1-Tq^{-1}(1-h/\ell ))(1-hT^{-1})\left( \mathrm{E}%
\left[ \nu _{1,1,h}\right] +\mathrm{E}\left[ \nu _{1,1+h,-h}\right] \right) .
\label{P_B_L1_d_13}
\end{eqnarray}%
By the triangle inequality, for any $k,k^{\prime }\leq d$, we have:%
\begin{eqnarray}
&&\left \vert \sum_{h=0}^{\ell -1}\left( 1-Tq^{-1}(1-h/\ell )\right)
(1-hT^{-1})\mathrm{E}\left[ \nu _{1,1,h}(k,k^{\prime })\right] \right \vert 
\notag \\
&\leq &(Tq^{-1}-1)\sum_{h=0}^{\ell -1}\mathrm{E}\left[ |\nu
_{1,1,h}(k,k^{\prime })|\right] +Tq^{-1}\ell ^{-1}\sum_{h=0}^{\ell -1}h%
\mathrm{E}\left[ |\nu _{1,1,h}(k,k^{\prime })|\right]  \notag \\
&\leq &C\ell T^{-1}\sum_{h=0}^{\ell -1}\alpha _{h}^{1-4/r}+C\ell
^{-1}\sum_{h=1}^{\ell -1}h\alpha _{h}^{1-4/r}\leq C(\ell T^{-1}+\ell ^{-1}),
\label{P_B_L1_d_14}
\end{eqnarray}%
where the second inequality is by (\ref{P_B_L1_d_6}), and the last
inequality is by Assumption \ref{A1}(i). Similarly, we can show that 
\begin{equation}
\left \vert \sum_{h=1}^{\ell -1}\left( 1-Tq^{-1}(1-h/\ell )\right)
(1-hT^{-1})\mathrm{E}\left[ \nu _{1,1+h,-h}(k,k^{\prime })\right] \right
\vert \leq C(\ell T^{-1}+\ell ^{-1})  \label{P_B_L1_d_15}
\end{equation}%
and%
\begin{equation}
\left \vert \sum_{h=\ell }^{T-1}(1-hT^{-1})\left( \mathrm{E}\left[ \nu
_{1,1,h}(k,k^{\prime })\right] +\mathrm{E}\left[ \nu _{1,1+h,-h}(k,k^{\prime
})\right] \right) \right \vert \leq C\sum_{h=\ell }^{T-1}\alpha
_{h}^{1-4/r}\leq C\ell ^{-1}.  \label{P_B_L1_d_16}
\end{equation}%
The desired result in (\ref{P_B_L1_d_8}) now follows from (\ref{P_B_L1_d_12}%
) and (\ref{P_B_L1_d_13})-(\ref{P_B_L1_d_16}).\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L1_da}\ Under Assumptions \ref{A1} and \ref{A2},\ we have:%
\begin{eqnarray*}
&&\mathrm{Cov}\left( T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t},T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i^{\prime },t}\varepsilon
_{i^{\prime },t}\right) \\
&=&\lim_{T\rightarrow \infty }\mathrm{Cov}\left( T^{-1/2}\sum_{t\leq T}%
\tilde{R}_{-i,t}\varepsilon _{i,t},T^{-1/2}\sum_{t\leq T}\tilde{R}%
_{-i^{\prime },t}\varepsilon _{i^{\prime },t}\right) +O(T^{-1}).
\end{eqnarray*}
\end{lemma}

\noindent \textsc{Proof.} Recall that\ $\nu _{1,t,h}\equiv \tilde{R}_{-i,t}%
\tilde{R}_{-i^{\prime },t+h}^{\top }\varepsilon _{i,t}\varepsilon
_{i^{\prime },t+h}$. In view of the expression in\ (\ref{P_B_L1_d_12b}), the
claim of the lemma follows if for any $k,k^{\prime }\leq d$: 
\begin{equation}
\sum_{h=1}^{T-1}\left \vert h\left( \mathrm{E}\left[ \nu
_{1,1,h}(k,k^{\prime })\right] +\mathrm{E}\left[ \nu _{1,1+h,-h}(k,k^{\prime
})\right] \right) \right \vert \leq C  \label{P_B_L1_da_1}
\end{equation}%
and%
\begin{equation}
\sum_{h=T}^{\infty }\left \vert \mathrm{E}\left[ \nu _{1,1,h}(k,k^{\prime })%
\right] +\mathrm{E}\left[ \nu _{1,1+h,-h}(k,k^{\prime })\right] \right \vert
\leq CT^{-1},  \label{P_B_L1_da_2}
\end{equation}%
where\ $\nu _{1,1,h}(k,k^{\prime })$ denotes the entry of $\nu _{1,t,h}$ on
its $k$-th row and $k^{\prime }$-th column.\ By\ (\ref{P_B_L1_d_6}) and
Assumption \ref{A1}(i),\ we obtain 
\begin{equation}
\sum_{h=1}^{T-1}\left \vert h\left( \mathrm{E}\left[ \nu
_{1,1,h}(k,k^{\prime })\right] +\mathrm{E}\left[ \nu _{1,1+h,-h}(k,k^{\prime
})\right] \right) \right \vert \leq C\sum_{h=1}^{T-1}h\alpha
_{h}^{1-4/r}\leq C.  \label{P_B_L1_da_3}
\end{equation}%
Similarly, 
\begin{equation}
\sum_{h=T}^{\infty }\left \vert \mathrm{E}\left[ \nu _{1,1,h}(k,k^{\prime })%
\right] +\mathrm{E}\left[ \nu _{1,1+h,-h}(k,k^{\prime })\right] \right \vert
\leq C\sum_{h=T}^{\infty }\alpha _{h}^{1-4/r}\leq CT^{-1}.
\label{P_B_L1_da_4}
\end{equation}%
The desired result in (\ref{P_B_L1_da_1}) and (\ref{P_B_L1_da_2}) follow
from (\ref{P_B_L1_da_3}) and (\ref{P_B_L1_da_4}), respectively.

\bigskip

\begin{lemma}
\label{B_L1_e} Under\ Assumptions \ref{A1} and \ref{A2}, we have wpa1:\ (i) $%
q^{-1}\sum_{j\leq q}||\ell ^{-1}\sum_{l\leq \ell }\tilde{R}_{j+l-1}\tilde{R}%
_{j+l-1}^{\top }||^{2}\leq C$; and (ii) $\lambda _{\min }^{-1}(\hat{Q}_{\ell
})+\lambda _{\max }(\hat{Q}_{\ell })\leq C$, where $\hat{Q}_{\ell }\equiv
\ell ^{-1}\sum_{t<\ell }(\tilde{R}_{t}\tilde{R}_{t}^{\top }+\tilde{R}_{T-t+1}%
\tilde{R}_{T-t+1}^{\top })$.
\end{lemma}

\noindent \textsc{Proof.} (i) By the triangle inequality, we have 
\begin{eqnarray}
\left \Vert \ell ^{-1}\sum_{l\leq \ell }\tilde{R}_{j+l-1}\tilde{R}%
_{j+l-1}^{\top }\right \Vert ^{2} &\leq &\left \Vert \mathrm{E}[\tilde{R}%
_{j+l-1}\tilde{R}_{j+l-1}^{\top }]\right \Vert ^{2}  \notag \\
&&+\left \Vert \ell ^{-1}\sum_{l\leq \ell }(\tilde{R}_{j+l-1}\tilde{R}%
_{j+l-1}^{\top }-\mathrm{E}[\tilde{R}_{j+l-1}\tilde{R}_{j+l-1}^{\top
}])\right \Vert ^{2}.  \label{P_B_L1_e_1}
\end{eqnarray}%
Under (\ref{P_I_L1_5}), the first term on the right-hand side of inequality (%
\ref{P_B_L1_e_1}) can be bounded as:%
\begin{equation}
q^{-1}\sum_{j\leq q}\left \Vert \mathrm{E}[\tilde{R}_{j+l-1}\tilde{R}%
_{j+l-1}^{\top }]\right \Vert ^{2}\leq Cq^{-1}\sum_{j\leq q}(\lambda _{\max
}(Q))^{2}\leq C.  \label{P_B_L1_e_2}
\end{equation}%
Using similar arguments as in the proofs of (\ref{P_I_L1_1b}) and (\ref%
{P_I_L1_3}), we can show: 
\begin{equation*}
\sum_{j\leq q}\mathrm{E}\left[ \left \Vert \ell ^{-1}\sum_{l\leq \ell }(%
\tilde{R}_{j+l-1}\tilde{R}_{j+l-1}^{\top }-\mathrm{E}[\tilde{R}_{j+l-1}%
\tilde{R}_{j+l-1}^{\top }])\right \Vert ^{2}\right] \leq C\sum_{j\leq q}\ell
^{-1}\leq Cq\ell ^{-1},
\end{equation*}%
which, together with Markov's inequality, implies that 
\begin{equation}
q^{-1}\sum_{j\leq q}\left \Vert \ell ^{-1}\sum_{l\leq \ell }(\tilde{R}%
_{j+l-1}\tilde{R}_{j+l-1}^{\top }-\mathrm{E}[\tilde{R}_{j+l-1}\tilde{R}%
_{j+l-1}^{\top }])\right \Vert ^{2}=O_{p}(\ell ^{-1}).  \label{P_B_L1_e_3}
\end{equation}%
Since\ $\ell \rightarrow \infty $ as the sample size increases, the claim in
part (i) of the lemma follows from\ (\ref{P_B_L1_e_1}), (\ref{P_B_L1_e_2})
and (\ref{P_B_L1_e_3}).

(ii)\ Using the same arguments as those in the proof of Lemma \ref{I_L1}(i),
we obtain the following: 
\begin{equation}
\ell ^{-1}\sum_{t<\ell }(\tilde{R}_{t}\tilde{R}_{t}^{\top }+\tilde{R}_{T-t+1}%
\tilde{R}_{T-t+1}^{\top }-\mathrm{E}[\tilde{R}_{t}\tilde{R}_{t}^{\top }+%
\tilde{R}_{T-t+1}\tilde{R}_{T-t+1}^{\top }])=O_{p}(\ell ^{-1/2}).
\label{P_B_L1_e_4}
\end{equation}%
Since\ $\ell \rightarrow \infty $ as the sample size increases, the claim in
part (ii) of the lemma follows from\ (\ref{P_B_L1_e_4})\ and by applying
similar arguments as those used to prove (\ref{P_I_L1_12a}).\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L1_f} Under\ Assumptions \ref{A1} and \ref{A2},\ we have wpa1: (i) $%
\max_{i\leq d}\ell ^{-1}\sum_{t<\ell }(\varepsilon _{i,t}^{2}+\varepsilon
_{i,T-t+1}^{2})\leq C$; and (ii) $q^{-1}\sum_{j\leq q}(\ell ^{-1}\sum_{l\leq
\ell }\varepsilon _{i,j+l-1}^{2})^{2}\leq C$.
\end{lemma}

\noindent \textsc{Proof.} By the similar arguments for proving (\ref%
{P_I_L1_16}), we have%
\begin{equation*}
\max_{i\leq d}\left \vert \ell ^{-1}\sum_{t<\ell }(\varepsilon
_{i,t}^{2}-\sigma _{\varepsilon _{i}}^{2})\right \vert +\max_{i\leq d}\left
\vert \ell ^{-1}\sum_{t<\ell }(\varepsilon _{i,T-t+1}^{2}-\sigma
_{\varepsilon _{i}}^{2})\right \vert =O_{p}(\ell ^{-1/2})
\end{equation*}%
which, along with (\ref{P_I_L1_15b}) shows the claim in part (i) of the
lemma. Part (ii) of the lemma can be established using the similar arguments
for showing Lemma \ref{B_L1_e}(i), and hence its proof is omitted.\hfill $%
Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L1_g}\ Under\ Assumptions \ref{A1} and \ref{A2},\ we have $%
\max_{i\leq d}\mathrm{E}^{\ast }[||\sum_{l\leq \ell }\tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b}||^{3}]=O_{p}(\ell ^{3/2})$.
\end{lemma}

\noindent \textsc{Proof.} First, we note that 
\begin{equation}
\mathrm{E}^{\ast }\left[ \left \Vert \sum_{l\leq \ell }\tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b}\right \Vert ^{3}\right] =q^{-1}\sum_{j\leq
q}\left \Vert \sum_{l\leq \ell }\tilde{R}_{i^{\prime },j+l-1}\varepsilon
_{i,j+l-1}\right \Vert ^{3}.  \label{P_B_L1_g_1}
\end{equation}%
Applying Rosenthal's inequality of strong mixing processes (see, e.g.,
Theorem 2 in Section 1.4 of \cite{doukhan1994mixing}), we get%
\begin{equation}
\mathbb{E}\left[ \left \vert \sum_{l\leq \ell }\varepsilon _{i,j+l-1}\right
\vert ^{3}\right] \leq C\max \left \{ \left( \sum_{l\leq \ell }\left \Vert
\varepsilon _{i,j+l-1}\right \Vert _{2+\delta }^{2}\right)
^{3/2},\sum_{l\leq \ell }\left \Vert \varepsilon _{i,j+l-1}\right \Vert
_{3+\delta }^{3}\right \} \leq C\ell ^{3/2},  \label{P_B_L1_g_2}
\end{equation}%
where the second inequality is by (\ref{P_I_L1_15b}). Similarly for any $%
i^{\prime }\leq d$ with $i^{\prime }\neq i$, we can show that%
\begin{equation*}
\mathrm{E}\left[ \left \vert \sum_{l\leq \ell }R_{i^{\prime
},j+l-1}\varepsilon _{i,j+l-1}\right \vert ^{3}\right] \leq C\ell ^{3/2},
\end{equation*}%
which, together with (\ref{P_B_L1_g_2}), shows that 
\begin{equation}
q^{-1}\sum_{j\leq q}\mathrm{E}\left[ \left \Vert \sum_{l\leq \ell }\tilde{R}%
_{i^{\prime },j+l-1}\varepsilon _{i,j+l-1}\right \Vert ^{3}\right] \leq
C\ell ^{3/2}.  \label{P_B_L1_g_3}
\end{equation}%
The claim of the lemma follows from (\ref{P_B_L1_g_3}) and Markov's
inequality.\hfill $Q.E.D.$

\bigskip

Let $\mathcal{D}_{1,T}$ denote the subset of the sampling space such that:
(i) $||\hat{Q}-Q||\leq \log (T)^{1/2}T^{-1/2}$; (ii) $\lambda _{\min }^{-1}(%
\hat{Q}_{\ell })+\lambda _{\max }(\hat{Q}_{\ell })\leq C$; and (iii) $%
q^{-1}\sum_{j\leq q}||\ell ^{-1}\sum_{l\leq \ell }\tilde{R}_{j+l-1}\tilde{R}%
_{j+l-1}^{\top }||^{2}\leq C$. By Lemma \ref{I_L1}(i) and Lemma \ref{B_L1_e}%
, we have $\mathrm{P}\left( \mathcal{D}_{1,T}\right) \rightarrow 1$ as $%
T\rightarrow \infty $.

\begin{lemma}
\label{B_L2}\ Conditional on $\mathcal{D}_{1,T}$,\ for any finite constant $%
C_{1}$\ and any $c_{1}\in \lbrack 0,1/2)$ we have:%
\begin{equation*}
\mathrm{P}^{\ast }\left( ||\hat{Q}^{b}-\hat{Q}||>C_{1}(\ell
T^{-1})^{c_{1}}\right) \leq CC_{1}^{-2}(\ell T^{-1})^{1-2c_{1}}.
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} Applying Lemma\  \ref{B_L1_a}, we can write%
\begin{equation}
\mathrm{E}^{\ast }[\hat{Q}^{b}]-\hat{Q}=(Tq^{-1}-1)\hat{Q}%
-q^{-1}\sum_{t<\ell }(1-t/\ell )(\tilde{R}_{t}\tilde{R}_{t}^{\top }+\tilde{R}%
_{T-t+1}\tilde{R}_{T-t+1}^{\top }).  \label{P_B_L2_1}
\end{equation}%
Therefore, by the triangle inequality and conditional on $\mathcal{D}_{1,T}$%
, we have%
\begin{equation}
||\mathrm{E}^{\ast }[\hat{Q}^{b}]-\hat{Q}||\leq (Tq^{-1}-1)||\hat{Q}||+\ell
q^{-1}||\hat{Q}_{\ell }||\leq C\ell T^{-1}.  \label{P_B_L2_2}
\end{equation}%
Let $\hat{Q}_{j}^{b}\equiv \ell ^{-1}\sum_{l\leq \ell }\tilde{R}_{\ell
(j-1)+l}^{b}(\tilde{R}_{\ell (j-1)+l}^{b})^{\top }$. Since $Z_{j}^{b}\equiv (%
\tilde{R}_{(j-1)\ell +1}^{b},\ldots ,\tilde{R}_{j\ell }^{b})$ is i.i.d.
across $j$ given the data and $\hat{Q}^{b}=m^{-1}\sum_{j\leq m}\hat{Q}%
_{j}^{b}$,\ we have%
\begin{equation}
\mathrm{E}^{\ast }\left[ ||\hat{Q}^{b}-\mathrm{E}^{\ast }[\hat{Q}^{b}]||^{2}%
\right] =m^{-1}\mathrm{E}^{\ast }\left[ ||\hat{Q}_{1}^{b}-\mathrm{E}^{\ast }[%
\hat{Q}_{1}^{b}]||^{2}\right] \leq m^{-1}\mathrm{E}^{\ast }\left[ ||\hat{Q}%
_{1}^{b}||^{2}\right] .  \label{P_B_L2_3}
\end{equation}%
Next conditional on $\mathcal{D}_{1,T}$, we observe:%
\begin{equation}
\mathrm{E}^{\ast }\left[ ||\hat{Q}_{1}^{b}||^{2}\right] =q^{-1}\sum_{j\leq q}%
\left[ \left \Vert \ell ^{-1}\sum_{l\leq \ell }\tilde{R}_{j+l-1}\tilde{R}%
_{j+l-1}^{\top }\right \Vert ^{2}\right] \leq C.  \label{P_B_L2_4}
\end{equation}%
By the definition of $m$, it is clear that $m^{-1}\leq C\ell T^{-1}$.
Combining the results in\ (\ref{P_B_L2_3}) and\ (\ref{P_B_L2_4}), and
applying Markov's inequality, we obtain%
\begin{equation}
\mathrm{P}^{\ast }\left( ||\hat{Q}^{b}-\mathrm{E}^{\ast }[\hat{Q}%
^{b}]||>2^{-1}C_{1}(\ell T^{-1})^{c_{1}}\right) \leq CC_{1}^{-2}(\ell
T^{-1})^{1-2c_{1}}  \label{P_B_L2_5}
\end{equation}%
which, along with the triangle inequality and (\ref{P_B_L2_2}), shows that
for all large $T$:\ 
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \left \Vert \hat{Q}^{b}-\hat{Q}\right \Vert
>C_{1}(\ell T^{-1})^{c_{1}}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert \hat{Q}^{b}-\mathrm{E}^{\ast }[%
\hat{Q}^{b}]\right \Vert +\left \Vert \mathrm{E}^{\ast }[\hat{Q}^{b}]-\hat{Q}%
\right \Vert >C_{1}(\ell T^{-1})^{c_{1}}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert \hat{Q}^{b}-\mathrm{E}^{\ast }[%
\hat{Q}^{b}]\right \Vert >2^{-1}C_{1}(\ell T^{-1})^{c_{1}}\right) \leq
CC_{1}^{-2}(\ell T^{-1})^{1-2c_{1}},  \label{P_B_L2_6}
\end{eqnarray}%
conditional on $\mathcal{D}_{1,T}$. The claim of the lemma now follows from (%
\ref{P_B_L2_6}).\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L2b}\ Conditional on $\mathcal{D}_{1,T}$,\ we have%
\begin{equation*}
\mathrm{P}^{\ast }\left( \lambda _{\min }(\hat{Q})/2\leq \lambda _{\min }(%
\hat{Q}^{b})\leq \lambda _{\max }(\hat{Q}^{b})\leq 2\lambda _{\max }(\hat{Q}%
)\right) \geq 1-C\ell T^{-1}.
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} Since\ $\hat{Q}^{b}=\hat{Q}+(\hat{Q}^{b}-\hat{Q})$%
, it follows that 
\begin{equation}
\lambda _{\max }(\hat{Q}^{b})\leq \lambda _{\max }(\hat{Q})+\lambda _{\max }(%
\hat{Q}^{b}-\hat{Q})\leq \lambda _{\max }(\hat{Q})+||\hat{Q}^{b}-\hat{Q}||.
\label{P_B_L2b_1}
\end{equation}%
Thus,\ conditional on $\mathcal{D}_{1,T}$, we can apply\ Lemma \ref{B_L2}
(with $C_{1}=\lambda _{\max }(\hat{Q})$ and $c_{1}=0$), and (\ref{P_B_L2b_1}%
) to obtain: 
\begin{equation}
\mathrm{P}^{\ast }\left( \lambda _{\max }(\hat{Q}^{b})\leq 2\lambda _{\max }(%
\hat{Q})\right) \geq \mathrm{P}^{\ast }\left( ||\hat{Q}^{b}-\hat{Q}||\leq
\lambda _{\max }(\hat{Q})\right) \geq 1-C\ell T^{-1},  \label{P_B_L2b_2}
\end{equation}%
for all large $T$. Using similar arguments as those in the derivation of (%
\ref{P_B_L2b_1}), we have 
\begin{equation*}
\lambda _{\min }(\hat{Q}^{b})\geq \lambda _{\min }(\hat{Q})-||\hat{Q}^{b}-%
\hat{Q}||,
\end{equation*}%
which, combined with Lemma \ref{B_L2}\ (with $C_{1}=\lambda _{\min }(\hat{Q}%
)/2$ and $c_{1}=0$), implies that conditional on $\mathcal{D}_{1,T}$, we
obtain 
\begin{equation}
\mathrm{P}^{\ast }\left( \lambda _{\min }(\hat{Q}^{b})\geq \lambda _{\min }(%
\hat{Q})/2\right) \geq \mathrm{P}^{\ast }\left( ||\hat{Q}^{b}-\hat{Q}||\leq
\lambda _{\min }(\hat{Q})/2\right) \geq 1-C\ell T^{-1},  \label{P_B_L2b_3}
\end{equation}%
for all large $T$. Therefore, combining the results in\ (\ref{P_B_L2b_2})
and (\ref{P_B_L2b_3}), and conditional on $\mathcal{D}_{1,T}$, we obtain%
\begin{eqnarray*}
&&\mathrm{P}^{\ast }\left( \lambda _{\min }(\hat{Q})/2\leq \lambda _{\min }(%
\hat{Q}^{b})\leq \lambda _{\max }(\hat{Q}^{b})\leq 2\lambda _{\max }(\hat{Q}%
)\right) \\
&\geq &\mathrm{P}^{\ast }\left( \lambda _{\max }(\hat{Q}^{b})\leq 2\lambda
_{\max }(\hat{Q})\right) +\mathrm{P}^{\ast }\left( \lambda _{\min }(\hat{Q}%
^{b})\geq \lambda _{\min }(\hat{Q})/2\right) -1\geq 1-C\ell T^{-1},
\end{eqnarray*}%
which establishes the claim of the lemma.\hfill $Q.E.D.$

\bigskip

By the triangle inequality, Assumption \ref{A2}(ii),\ Lemma \ref{I_L1}(ii)
and Lemma \ref{B_L1_c}, it follows that:%
\begin{equation}
\left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }[\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}]\right \Vert =O_{p}(T^{-1/2}).
\label{D_2T_1}
\end{equation}%
Since\ $||\mathrm{Var}(T^{-1/2}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon
_{i,t})||\leq C$ by (\ref{P_I_L3_5}), from Lemma \ref{B_L1_d} we have wpa1: 
\begin{equation}
\left \Vert \mathrm{Var}^{\ast }\left( (m\ell )^{-1/2}\sum_{t\leq m\ell }%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right) \right \Vert \leq C.
\label{D_2T_2}
\end{equation}%
Let\ $\mathcal{D}_{2,T}^{0}$ be the subset of the sampling space such that:
(i) $||(m\ell )^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }[\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}]||\leq (\log (T)/T)^{1/2}$; and (ii) (\ref%
{D_2T_2}) holds. From the discussion above, it is clear that $\mathrm{P}%
\left( \mathcal{D}_{2,T}\right) \rightarrow 1$ as $T\rightarrow \infty $,
where $\mathcal{D}_{2,T}\equiv \mathcal{D}_{1,T}\cap \mathcal{D}_{2,T}^{0}$.

\begin{lemma}
\label{B_L3}\ Conditional on $\mathcal{D}_{2,T}$,\ for finite constant $%
C_{2} $\ and any $c_{2}\in (0,1/2)$ we have: 
\begin{equation*}
\mathrm{P}^{\ast }\left( \max_{i\leq d}\left( |\hat{\alpha}_{i}^{b}-\alpha
_{i}|^{2}+||\hat{\beta}_{i}^{b}-\beta _{i}||^{2}\right) \geq
C_{2}T^{-2c_{2}}\right) \leq C(C_{2}^{-2}T^{-1+2c_{2}}+\ell T^{-1}).
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} Let $\varepsilon _{i,t}^{b}\equiv
R_{i,t}^{b}-\alpha _{i}-\beta _{i}^{\top }\tilde{R}_{-i,t}^{b}$. Then by the
definition of $\hat{\alpha}_{i}^{b}$ and $\hat{\beta}_{i}^{b}$, it follows
that%
\begin{equation}
|\hat{\alpha}_{i}^{b}-\alpha _{i}|^{2}+||\hat{\beta}_{i}^{b}-\beta
_{i}||^{2}=\left \Vert \frac{(\hat{Q}_{-i}^{b})^{-1}}{m\ell }\sum_{t\leq
m\ell }\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right \Vert ^{2}\leq \frac{%
\left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }\tilde{R}_{-i,t}^{b}\varepsilon
_{i,t}^{b}\right \Vert ^{2}}{(\lambda _{\min }(\hat{Q}^{b}))^{2}}.
\label{P_B_L3_1}
\end{equation}%
Conditional on $\mathcal{D}_{2,T}$, we can use the triangle inequality and
Markov's inequality to deduce that: 
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right \Vert >\tilde{C}%
_{2}T^{-c_{2}}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }(%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}-\mathrm{E}^{\ast }[\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}])\right \Vert +\left \Vert (m\ell
)^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }[\tilde{R}_{-i,t}^{b}\varepsilon
_{i,t}^{b}]\right \Vert >\tilde{C}_{2}T^{-c_{2}}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }(%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}-\mathrm{E}^{\ast }[\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}])\right \Vert >2^{-1}\tilde{C}%
_{2}T^{-c_{2}}\right) \leq C\tilde{C}_{2}^{-2}T^{-1+2c_{2}},
\label{P_B_L3_3}
\end{eqnarray}%
for any finite constant $\tilde{C}_{2}$\ and any $c_{2}\in (0,1/2)$.
Combining Lemma \ref{B_L2b} with (\ref{P_B_L3_1}) and (\ref{P_B_L3_3}) leads
to:%
\begin{eqnarray*}
&&\mathrm{P}^{\ast }\left( \max_{i\leq d}(|\hat{\alpha}_{i}^{b}-\alpha
_{i}|^{2}+||\hat{\beta}_{i}^{b}-\beta _{i}||^{2})\geq C_{2}T^{-2c_{2}}\right)
\\
&\leq &\mathrm{P}^{\ast }\left( \max_{i\leq d}\left \Vert (m\ell
)^{-1}\sum_{t\leq m\ell }\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right
\Vert ^{2}\geq C_{2}(\lambda _{\min }(\hat{Q}^{b}))^{2}T^{-2c_{2}}\right) \\
&\leq &\sum_{i\leq d}\mathrm{P}^{\ast }\left( \left \Vert (m\ell
)^{-1}\sum_{t\leq m\ell }\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right
\Vert \geq \frac{C_{2}\lambda _{\min }(\hat{Q})T^{-c_{2}}}{2}\right) +%
\mathrm{P}^{\ast }\left( \lambda _{\min }(\hat{Q}^{b})<\lambda _{\min }(\hat{%
Q})/2\right) \\
&\leq &C(C_{2}^{-2}T^{-1+2c_{2}}+\ell T^{-1}),
\end{eqnarray*}%
which shows the claim of the lemma.\hfill $Q.E.D.$

\bigskip

Let\ $\mathcal{D}_{3,T}^{0}$ denote the subset of the sampling space such
that: (i) $\max_{i\leq d}\left \vert \tilde{\sigma}_{\varepsilon
_{i}}^{2}-\sigma _{\varepsilon _{i}}^{2}\right \vert \leq \log
(T)^{1/2}T^{-1/2}$ where $\tilde{\sigma}_{\varepsilon _{i}}^{2}\equiv
T^{-1}\sum_{t\leq T}\varepsilon _{i,t}^{2}$;\ (ii) $\max_{i\leq d}\ell
^{-1}\sum_{t<\ell }(\varepsilon _{i,t}^{2}+\varepsilon _{i,T-t+1}^{2})\leq C$%
; and (iii) $q^{-1}\sum_{j\leq q}(\ell ^{-1}\sum_{l\leq \ell }\varepsilon
_{i,j+l-1}^{2})^{2}\leq C$.\ Then under $\mathcal{D}_{3,T}^{0}$, we can use (%
\ref{P_I_L1_15b}) and (\ref{P_I_L1_18}) in the proof of Lemma \ref{I_L1b} to
obtain%
\begin{equation*}
C^{-1}\leq \min_{i\leq d}\tilde{\sigma}_{\varepsilon _{i}}^{2}\leq
\max_{i\leq d}\tilde{\sigma}_{\varepsilon _{i}}^{2}\leq C,
\end{equation*}%
wpa1. Furthermore, by (\ref{P_I_L1_16}) and Lemma \ref{B_L1_f}, and the
property of $\mathcal{D}_{2,T}$, we have $\mathrm{P}\left( \mathcal{D}%
_{3,T}\right) \rightarrow 1$ as $T\rightarrow \infty $, where $\mathcal{D}%
_{3,T}\equiv \mathcal{D}_{2,T}\cap \mathcal{D}_{3,T}^{0}$.

\begin{lemma}
\label{B_L4a} Conditional on $\mathcal{D}_{3,T}$, for any finite constant $%
C_{3}$\ and any $c_{3}\in (0,1/2)$ we have 
\begin{equation*}
\mathrm{P}^{\ast }\left( \max_{i\leq d}\max_{j=1,2}|(\hat{\sigma}%
_{\varepsilon _{i}}^{b})^{2}-\sigma _{\varepsilon _{i}}^{2}|\geq C_{3}(\ell
T^{-1})^{c_{3}}\right) \leq CC_{3}^{-2}(\ell T^{-1})^{1-2c_{3}}.
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} Since $\hat{\varepsilon}_{i,t}^{b}=\varepsilon
_{i,t}^{b}-(\hat{\alpha}_{i}^{b}-\alpha _{i},(\hat{\beta}_{i}^{b}-\beta
_{i})^{\top })\tilde{R}_{-i,t}^{b}$, we can write 
\begin{eqnarray}
(\hat{\sigma}_{\varepsilon _{i}}^{b})^{2} &=&(m\ell )^{-1}\sum_{t\leq m\ell
}(\varepsilon _{i,t}^{b})^{2}-2(\hat{\alpha}_{i}^{b}-\alpha _{i},(\hat{\beta}%
_{i}^{b}-\beta _{i})^{\top })(m\ell )^{-1}\sum_{t\leq m\ell }\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}  \notag \\
&&+(\hat{\alpha}_{i}^{b}-\alpha _{i},(\hat{\beta}_{i}^{b}-\beta _{i})^{\top
})\hat{Q}_{-i}^{b}(\hat{\alpha}_{i}^{b}-\alpha _{i},(\hat{\beta}%
_{i}^{b}-\beta _{i})^{\top })^{\top }.  \label{P_B_L4a_1}
\end{eqnarray}%
By the Cauchy-Schwarz inequality, Lemma \ref{B_L3} and (\ref{P_B_L3_3}), and
conditional on $\mathcal{D}_{3,T}$, we have: 
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \left \vert (\hat{\alpha}_{i}^{b}-\alpha _{i},(%
\hat{\beta}_{i}^{b}-\beta _{i})^{\top })(m\ell )^{-1}\sum_{t\leq m\ell }%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right \vert \geq
T^{-2c_{3}}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert (\hat{\alpha}_{i}^{b}-\alpha
_{i},(\hat{\beta}_{i}^{b}-\beta _{i})^{\top })\right \Vert \left \Vert
(m\ell )^{-1}\sum_{t\leq m\ell }\tilde{R}_{-i,t}^{b}\varepsilon
_{i,t}^{b}\right \Vert \geq T^{-2c_{3}}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right \Vert \geq
T^{-c_{3}}\right) +\mathrm{P}^{\ast }\left( \left \Vert (\hat{\alpha}%
_{i}^{b}-\alpha _{i},(\hat{\beta}_{i}^{b}-\beta _{i})^{\top })\right \Vert
\geq T^{-c_{3}}\right)  \notag \\
&\leq &C(T^{-1+2c_{3}}+\ell T^{-1}).  \label{P_B_L4a_2}
\end{eqnarray}%
Similarly, by Lemmas \ref{B_L2b} and \ref{B_L3}, and conditional on $%
\mathcal{D}_{3,T}$, we have%
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( (\hat{\alpha}_{i}^{b}-\alpha _{i},(\hat{\beta}%
_{i}^{b}-\beta _{i})^{\top })\hat{Q}_{-i}^{b}(\hat{\alpha}_{i}^{b}-\alpha
_{i},(\hat{\beta}_{i}^{b}-\beta _{i})^{\top })^{\top }\geq T^{-2c_{3}}\right)
\notag \\
&\leq &\mathrm{P}^{\ast }\left( \lambda _{\max }(\hat{Q}_{-i}^{b})\left
\Vert (\hat{\alpha}_{i}^{b}-\alpha _{i},(\hat{\beta}_{i}^{b}-\beta
_{i})^{\top })\right \Vert ^{2}\geq T^{-2c_{3}}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert (\hat{\alpha}_{i}^{b}-\alpha
_{i},(\hat{\beta}_{i}^{b}-\beta _{i})^{\top })\right \Vert ^{2}\geq \frac{%
T^{-2c_{3}}}{2\lambda _{\max }(\hat{Q})}\right) +C\ell T^{-1}\leq
C(T^{-1+2c_{3}}+\ell T^{-1}).  \label{P_B_L4a_3}
\end{eqnarray}

Next, we observe that by Lemma \ref{B_L1_a},%
\begin{equation}
(m\ell )^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }\left[ (\varepsilon
_{i,t}^{b})^{2}\right] -\tilde{\sigma}_{\varepsilon
_{i}}^{2}=(Tq^{-1}-1)T^{-1}\sum_{t\leq T}\varepsilon
_{i,t}^{2}-q^{-1}\sum_{t<\ell }(1-t/\ell )(\varepsilon
_{i,t}^{2}+\varepsilon _{i,T-t+1}^{2}).  \label{P_B_L4a_4}
\end{equation}%
Conditional on $\mathcal{D}_{3,T}$, we have 
\begin{equation}
\left \vert (m\ell )^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }\left[
(\varepsilon _{i,t}^{b})^{2}\right] -\tilde{\sigma}_{\varepsilon
_{i}}^{2}\right \vert \leq C\ell T^{-1},  \label{P_B_L4a_5}
\end{equation}%
and 
\begin{eqnarray}
\mathrm{Var}^{\ast }\left( (m\ell )^{-1}\sum_{t\leq m\ell }(\varepsilon
_{i,t}^{b})^{2}\right) &=&\mathrm{Var}^{\ast }\left( (m\ell
)^{-1}\sum_{j\leq m}\sum_{l\leq \ell }(\varepsilon _{i,\ell
(j-1)+l}^{b})^{2}\right)  \notag \\
&=&m^{-1}\mathrm{Var}^{\ast }\left( \ell ^{-1}\sum_{l\leq \ell }(\varepsilon
_{i,\ell (j-1)+l}^{b})^{2}\right) \leq m^{-1}\mathrm{E}^{\ast }\left[ \left(
\ell ^{-1}\sum_{l\leq \ell }(\varepsilon _{i,l}^{b})^{2}\right) ^{2}\right] 
\notag \\
&=&(mq)^{-1}\sum_{j\leq q}\left( \ell ^{-1}\sum_{l\leq \ell }\varepsilon
_{i,j+l-1}^{2}\right) ^{2}\leq C\ell T^{-1}.  \label{P_B_L4a_5b}
\end{eqnarray}%
Therefore, by\ Markov's inequality, (\ref{P_B_L4a_5}) and (\ref{P_B_L4a_5b}%
), and conditional on $\mathcal{D}_{T}$, we obtain:%
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \left \vert (m\ell )^{-1}\sum_{t\leq m\ell
}(\varepsilon _{i,t}^{b})^{2}-\tilde{\sigma}_{\varepsilon _{i}}^{2}\right
\vert \geq \frac{C_{3}(\ell T^{-1})^{c_{3}}}{2}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \vert (m\ell )^{-1}\sum_{t\leq m\ell
}((\varepsilon _{i,t}^{b})^{2}-\mathrm{E}^{\ast }[(\varepsilon
_{i,t}^{b})^{2}])\right \vert \geq \frac{C_{3}(\ell T^{-1})^{c_{3}}}{4}%
\right) \leq CC_{3}^{-2}(\ell T^{-1})^{1-2c_{3}}  \label{P_B_L4a_6}
\end{eqnarray}%
for all large $T$.\ Collecting the results in (\ref{P_B_L4a_1}), (\ref%
{P_B_L4a_2}), (\ref{P_B_L4a_3}) and (\ref{P_B_L4a_6}), we conclude that:%
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( |(\hat{\sigma}_{\varepsilon _{i}}^{b})^{2}-\tilde{%
\sigma}_{\varepsilon _{i}}^{2}|\geq C_{3}(\ell T^{-1})^{c_{3}}\right)  \notag
\\
&\leq &\mathrm{P}^{\ast }\left( \left \vert (m\ell )^{-1}\sum_{t\leq m\ell
}(\varepsilon _{i,t}^{b})^{2}-\tilde{\sigma}_{\varepsilon _{i}}^{2}\right
\vert \geq 2^{-1}C_{3}(\ell T^{-1})^{c_{3}}\right)  \notag \\
&&+\mathrm{P}^{\ast }\left( \left \vert (\hat{\alpha}_{i}^{b}-\alpha _{i},(%
\hat{\beta}_{i}^{b}-\beta _{i})^{\top })^{\top }(m\ell )^{-1}\sum_{t\leq
m\ell }\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right \vert
<T^{-2c_{3}}\right)  \notag \\
&&+\mathrm{P}^{\ast }\left( (\hat{\alpha}_{i}^{b}-\alpha _{i},(\hat{\beta}%
_{i}^{b}-\beta _{i})^{\top })^{\top }\hat{Q}_{-i}^{b}(\hat{\alpha}%
_{i}^{b}-\alpha _{i},(\hat{\beta}_{i}^{b}-\beta _{i})^{\top
}<T^{-2c_{3}}\right)  \notag \\
&\leq &C(C_{3}^{-2}(\ell T^{-1})^{1-2c_{3}}+\ell T^{-1})\leq
CC_{3}^{-2}(\ell T^{-1})^{1-2c_{3}}.  \label{P_B_L4a_7}
\end{eqnarray}%
Since $\max_{i\leq d}\left \vert \tilde{\sigma}_{\varepsilon
_{i}}^{2}-\sigma _{\varepsilon _{i}}^{2}\right \vert \leq \log
(T)^{1/2}T^{-1/2}$ under\ $\mathcal{D}_{3,T}$, this together with\ (\ref%
{P_B_L4a_7}), shows the claim of the lemma.\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L4}\ Conditional on $\mathcal{D}_{3,T}$, for any finite constant $%
C_{4}$ and any $c_{4}\in (0,1/2)$ we have%
\begin{equation*}
\mathrm{P}^{\ast }\left( \max_{i\leq d}\max_{j=1,2}|(\hat{s}%
_{i,j}^{b})^{2}/s_{i,j}^{2}-1|\geq C_{4}(\ell T^{-1})^{c_{4}}\right) \leq
CC_{4}^{-2}(\ell T^{-1})^{1-2c_{4}}.
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} By the triangle inequality, we have:%
\begin{equation}
\left \vert \frac{(\hat{s}_{i,j}^{b})^{2}}{s_{i,j}^{2}}-1\right \vert \leq 
\frac{\left \vert (\hat{\sigma}_{\varepsilon _{i}}^{b})^{2}-\sigma
_{\varepsilon _{i}}^{2}\right \vert A_{j,\cdot }(\hat{Q}_{-i}^{b})^{-1}A_{j,%
\cdot }^{\top }}{\sigma _{\varepsilon _{i}}^{2}A_{j,\cdot
}Q_{-i}^{-1}A_{j,\cdot }^{\top }}+\frac{|A_{j,\cdot }((\hat{Q}%
_{-i}^{b})^{-1}-Q_{-i}^{-1})A_{j,\cdot }^{\top }|}{A_{j,\cdot
}Q_{-i}^{-1}A_{j,\cdot }^{\top }}.  \label{P_B_L4_1}
\end{equation}%
From Lemmas \ref{B_L2b} and \ref{B_L4a}, conditional on\ $\mathcal{D}_{3,T}$%
, we obtain%
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \left \vert \frac{\left \vert (\hat{\sigma}%
_{\varepsilon _{i}}^{b})^{2}-\sigma _{\varepsilon _{i}}^{2}\right \vert
A_{j,\cdot }(\hat{Q}_{-i}^{b})^{-1}A_{j,\cdot }^{\top }}{\sigma
_{\varepsilon _{i}}^{2}A_{j,\cdot }Q_{-i}^{-1}A_{j,\cdot }^{\top }}\right
\vert \geq \frac{C_{4}(\ell T^{-1})^{c_{4}}}{2}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \frac{\lambda _{\max }(Q)}{\sigma
_{\varepsilon _{i}}^{2}\lambda _{\min }(\hat{Q}^{b})}\left \vert (\hat{\sigma%
}_{\varepsilon _{i}}^{b})^{2}-\sigma _{\varepsilon _{i}}^{2}\right \vert
\geq \frac{C_{4}(\ell T^{-1})^{c_{4}}}{2}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \vert (\hat{\sigma}_{\varepsilon
_{i}}^{b})^{2}-\sigma _{\varepsilon _{i}}^{2}\right \vert \geq \frac{%
C_{4}\lambda _{\min }(\hat{Q})\sigma _{\varepsilon _{i}}^{2}}{4\lambda
_{\max }(Q)}(\ell T^{-1})^{c_{4}}\right) +C\ell T^{-1}\leq CC_{4}^{-2}(\ell
T^{-1})^{1-2c_{4}}  \label{P_B_L4_2}
\end{eqnarray}%
for all large $T$. Similarly,\ by Lemmas \ref{B_L2} and \ref{B_L2b},
conditional on $\mathcal{D}_{3,T}$, we get%
\begin{eqnarray*}
&&\mathrm{P}^{\ast }\left( \left \vert \frac{|A_{j,\cdot }((\hat{Q}%
_{-i}^{b})^{-1}-Q_{-i}^{-1})A_{j,\cdot }^{\top }|}{A_{j,\cdot
}Q_{-i}^{-1}A_{j,\cdot }^{\top }}\right \vert \geq \frac{C_{4}(\ell
T^{-1})^{c_{4}}}{2}\right) \\
&\leq &\mathrm{P}^{\ast }\left( \frac{\lambda _{\max }(Q)}{\lambda _{\min }(%
\hat{Q}^{b})\lambda _{\min }(Q)}||\hat{Q}^{b}-Q||\geq \frac{C_{4}(\ell
T^{-1})^{c_{4}}}{2}\right) \\
&\leq &\mathrm{P}^{\ast }\left( ||\hat{Q}^{b}-\hat{Q}||\geq \frac{%
C_{4}\lambda _{\min }(Q)\lambda _{\min }(\hat{Q})}{4\lambda _{\max }(Q)}%
(\ell T^{-1})^{c_{4}}\right) +C\ell T^{-1}\leq CC_{4}^{-2}(\ell
T^{-1})^{1-2c_{4}}.
\end{eqnarray*}%
Combining this with (\ref{P_B_L4_1}) and (\ref{P_B_L4_2}), we conclude that%
\begin{eqnarray*}
&&\mathrm{P}^{\ast }\left( \max_{i\leq d}\max_{j=1,2}\left \vert \frac{(\hat{%
s}_{i,j}^{b})^{2}}{s_{i,j}^{2}}-1\right \vert >C_{4}(\ell
T^{-1})^{c_{4}}\right) \\
&\leq &\sum_{i\leq d}\sum_{j=1,2}\mathrm{P}^{\ast }\left( \frac{\left \vert (%
\hat{\sigma}_{\varepsilon _{i}}^{b})^{2}-\sigma _{\varepsilon
_{i}}^{2}\right \vert A_{j,\cdot }(\hat{Q}_{-i}^{b})^{-1}A_{j,\cdot }^{\top }%
}{\sigma _{\varepsilon _{i}}^{2}A_{j,\cdot }Q_{-i}^{-1}A_{j,\cdot }^{\top }}%
\geq \frac{C_{4}(\ell T^{-1})^{c_{4}}}{2}\right) \\
&&+\sum_{i\leq d}\sum_{j=1,2}\mathrm{P}^{\ast }\left( \frac{|A_{j,\cdot }((%
\hat{Q}_{-i}^{b})^{-1}-Q_{-i}^{-1})A_{j,\cdot }^{\top }|}{A_{j,\cdot
}Q_{-i}^{-1}A_{j,\cdot }^{\top }}\geq \frac{C_{4}(\ell T^{-1})^{c_{4}}}{2}%
\right) \\
&\leq &CC_{4}^{-2}(\ell T^{-1})^{1-2c_{4}},
\end{eqnarray*}%
which establishes the claim of the lemma.\hfill $Q.E.D.$

\bigskip

Recall that $e_{t}^{b}\equiv (e_{i,t}^{b})_{i\leq d}$, where $%
e_{i,t}^{b}\equiv (e_{i,j,t}^{b})_{j=1,2}$ and $e_{i,j,t}^{b}\equiv
A_{j,\cdot }Q_{-i}^{-1}(\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}-\mathrm{E}%
^{\ast }[\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}])$. Let\ $\mathcal{D}%
_{4,T}^{0}$ denote the subset of the sampling space such that: (i) $||\Omega
_{T}^{\ast }-\Omega _{d}||\leq \log (T)^{1/4}(\ell ^{2}T^{-1+2/\tilde{r}%
}+\ell ^{-1})$ where $\Omega _{T}^{\ast }\equiv \mathrm{Var}^{\ast }((m\ell
)^{-1/2}\sum_{t\leq m\ell }e_{t}^{b})$; (ii)%
\begin{equation*}
\left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }[\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}]-T^{-1}\sum_{t\leq T}\tilde{R}%
_{-i,t}\varepsilon _{i,t}\right \Vert \leq \log (T)^{1/2}\ell ^{1/2}T^{-1};
\end{equation*}%
and (ii) $\max_{i\leq d}\mathrm{E}^{\ast }[||\sum_{l\leq \ell }\tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b}||^{3}]\leq \log (T)^{1/2}\ell ^{3/2}$. By
Lemmas \ref{B_L1_c}, \ref{B_L1_d}, \ref{B_L1_da} and \ref{B_L1_g}, and the
properties of $\mathcal{D}_{3,T}$, we have $\mathrm{P}\left( \mathcal{D}%
_{4,T}\right) \rightarrow 1$ as $T\rightarrow \infty $, where $\mathcal{D}%
_{4,T}\equiv \mathcal{D}_{3,T}\cap \mathcal{D}_{4,T}^{0}$.

\begin{lemma}
\label{B_L5}\ Conditional on $\mathcal{D}_{4,T}$, for any finite constant $%
C_{5}$ and any\ $c_{5}\in (1/3,1/2)$ we have: 
\begin{equation*}
\mathrm{P}^{\ast }\left( \left \vert \frac{T^{1/2}(\hat{\theta}_{i,j}^{b}-%
\hat{\theta}_{i,j})}{\hat{s}_{i,j}^{b}}-\frac{(m\ell )^{-1/2}\sum_{t\leq
m\ell }e_{i,j,t}^{b}}{\hat{s}_{i,j}^{b}}\right \vert \geq C_{5}\ell
^{c_{5}}T^{-2c_{5}+1/2}\right) \leq C(\ell T^{-1})^{1-2c_{5}}.
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} By the definition of $\hat{\theta}_{i,j}^{b}$ and $%
\hat{\theta}_{i,j}$, we can write%
\begin{eqnarray}
\hat{\theta}_{i,j}^{b}-\hat{\theta}_{i,j} &=&A_{j,\cdot }((\hat{Q}%
_{-i}^{b})^{-1}-\hat{Q}_{-i}^{-1})\left( (m\ell )^{-1}\sum_{t\leq m\ell }%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right)  \notag \\
&&+A_{j,\cdot }\hat{Q}_{-i}^{-1}\left( (m\ell )^{-1}\sum_{t\leq m\ell }%
\mathrm{E}^{\ast }[\tilde{R}_{-i,t}^{b}\varepsilon
_{i,t}^{b}]-T^{-1}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}\right) 
\notag \\
&&+A_{j,\cdot }\hat{Q}_{-i}^{-1}\left( (m\ell )^{-1}\sum_{t\leq m\ell }(%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}-\mathrm{E}^{\ast }[\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}])\right) .  \label{P_B_L5_1}
\end{eqnarray}

Conditional on $\mathcal{D}_{4,T}$, we have%
\begin{equation}
\frac{\left \vert A_{j,\cdot }\hat{Q}_{-i}^{-1}\left( (m\ell
)^{-1}\sum_{t\leq m\ell }\mathrm{E}^{\ast }[\tilde{R}_{-i,t}^{b}\varepsilon
_{i,t}^{b}]-T^{-1}\sum_{t\leq T}\tilde{R}_{-i,t}\varepsilon _{i,t}\right)
\right \vert }{s_{i,j}}\leq C\log (T)^{1/2}\ell ^{1/2}T^{-1}.
\label{P_B_L5_2}
\end{equation}%
By the Cauchy-Schwarz inequality,%
\begin{eqnarray*}
&&\frac{\left \vert A_{j,\cdot }((\hat{Q}_{-i}^{b})^{-1}-\hat{Q}%
_{-i}^{-1})(m\ell )^{-1}\sum_{t\leq m\ell }\tilde{R}_{-i,t}^{b}\varepsilon
_{i,t}^{b}\right \vert }{s_{i,j}} \\
&\leq &\frac{\lambda _{\max }(Q)^{1/2}}{\sigma _{\varepsilon
_{i}}^{2}\lambda _{\min }(\hat{Q}^{b})\lambda _{\min }(\hat{Q})}||\hat{Q}%
^{b}-\hat{Q}||\left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}\right \Vert .
\end{eqnarray*}%
This, combined with Lemma \ref{B_L2}, implies that conditional on $\mathcal{D%
}_{4,T}$, we have 
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \frac{\left \vert A_{j,\cdot }((\hat{Q}%
_{-i}^{b})^{-1}-\hat{Q}_{-i}^{-1})(m\ell )^{-1}\sum_{t\leq m\ell }\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}\right \vert }{s_{i,j}}\geq \frac{(\ell
T^{-2})^{c_{5}}}{6}\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( ||\hat{Q}^{b}-\hat{Q}||\left \Vert (m\ell
)^{-1}\sum_{t\leq m\ell }\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right
\Vert \geq \frac{\sigma _{\varepsilon _{i}}^{2}(\lambda _{\min }(\hat{Q}%
))^{2}(\ell T^{-2})^{c_{5}}}{12\lambda _{\max }(Q)^{1/2}}\right) +C\ell
T^{-1}  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \Vert (m\ell )^{-1}\sum_{t\leq m\ell }%
\tilde{R}_{-i,t}^{b}\varepsilon _{i,t}^{b}\right \Vert \geq
T^{-c_{5}}\right) +C(\ell T^{-1})^{1-2c_{5}}\leq C(\ell T^{-1})^{1-2c_{5}},
\label{P_B_L5_3}
\end{eqnarray}%
where the last inequality is by (\ref{P_B_L3_3}).

Let $I_{1,n}^{b}\equiv s_{i,j}^{-1}|A_{j,\cdot }(\hat{Q}%
_{-i}^{-1}-Q_{-i}^{-1})((m\ell )^{-1/2}\sum_{t\leq m\ell }(\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}-\mathrm{E}^{\ast }[\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}]))|$. Then conditional on $\mathcal{D}%
_{4,T}$, we have 
\begin{equation*}
\mathrm{E}^{\ast }\left[ (I_{1,n}^{b})^{2}\right] \leq C\left \Vert \mathrm{%
Var}^{\ast }\left( (m\ell )^{-1/2}\sum_{t\leq m\ell }\tilde{R}%
_{-i,t}^{b}\varepsilon _{i,t}^{b}\right) \right \Vert ||\hat{Q}-Q||^{2}\leq
C\log (T)T^{-1},
\end{equation*}%
which together with Markov's inequality shows that 
\begin{equation}
\mathrm{P}^{\ast }\left( I_{1,n}^{b}\geq 6^{-1}C_{5}\ell
^{c_{5}}T^{-2c_{5}+1/2}\right) \leq C\log (T)\ell ^{-2c_{5}}T^{-2+4c_{5}}.
\label{P_B_L5_4}
\end{equation}%
This, along with (\ref{P_B_L5_1}), (\ref{P_B_L5_2}) and (\ref{P_B_L5_3}),
implies that%
\begin{equation}
\mathrm{P}^{\ast }\left( \frac{\left \vert T^{1/2}(\hat{\theta}_{i,j}^{b}-%
\hat{\theta}_{i,j})-(m\ell )^{-1/2}\sum_{t\leq m\ell }e_{i,j,t}^{b}\right
\vert }{s_{i,j}}\geq \frac{C_{5}\ell ^{c_{5}}T^{-2c_{5}+1/2}}{2}\right) \leq
C(\ell T^{-1})^{1-2c_{5}}.  \label{P_B_L5_6}
\end{equation}

Since $1+\hat{s}_{i,j}^{b}/s_{i,j}\geq 1$ conditional on $\mathcal{D}_{3,T}$%
, it follows that 
\begin{equation}
\left \vert \frac{\hat{s}_{i,j}^{b}}{s_{i,j}}-1\right \vert =\frac{\left
\vert (\hat{s}_{i,j}^{b})^{2}/s_{i,j}^{2}-1\right \vert }{\hat{s}%
_{i,j}^{b}/s_{i,j}+1}\leq \left \vert \frac{(\hat{s}_{i,j}^{b})^{2}}{%
s_{i,j}^{2}}-1\right \vert .  \label{P_B_L5_7A}
\end{equation}%
This, combining with Lemma \ref{B_L4}, implies that%
\begin{equation}
\mathrm{P}^{\ast }\left( \max_{i\leq d}\max_{j=1,2}\left \vert \frac{\hat{s}%
_{i,j}^{b}}{s_{i,j}}-1\right \vert \geq (\ell T^{-1})^{c_{5}}\right) \leq
C(\ell T^{-1})^{1-2c_{5}}.  \label{P_B_L5_7}
\end{equation}%
Thus, conditional on $\mathcal{D}_{3,T}$, we have:%
\begin{equation}
\mathrm{P}^{\ast }(1/2\leq \hat{s}_{i,j}^{b}/s_{i,j}\leq 2)\geq 1-C(\ell
T^{-1})^{1-2c_{5}}.  \label{P_B_L5_8}
\end{equation}%
From (\ref{P_B_L5_6}) and (\ref{P_B_L5_8}), we conclude that:%
\begin{eqnarray*}
&&\mathrm{P}^{\ast }\left( \frac{\left \vert T^{1/2}(\hat{\theta}_{i,j}^{b}-%
\hat{\theta}_{i,j})-(m\ell )^{-1/2}\sum_{t\leq m\ell }e_{i,j,t}^{b}\right
\vert }{\hat{s}_{i,j}^{b}}\geq C_{5}\ell ^{c_{5}}T^{-2c_{5}+1/2}\right) \\
&=&\mathrm{P}^{\ast }\left( \frac{\left \vert T^{1/2}(\hat{\theta}_{i,j}^{b}-%
\hat{\theta}_{i,j})-(m\ell )^{-1/2}\sum_{t\leq m\ell }e_{i,j,t}^{b}\right
\vert }{s_{i,j}}\geq C_{5}\frac{\hat{s}_{i,j}^{b}}{s_{i,j}}\ell
^{c_{5}}T^{-2c_{5}+1/2}\right) \\
&\leq &\mathrm{P}^{\ast }\left( \frac{\left \vert T^{1/2}(\hat{\theta}%
_{i,j}^{b}-\hat{\theta}_{i,j})-(m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{i,j,t}^{b}\right \vert }{s_{i,j}}\geq \frac{C_{5}\ell
^{c_{5}}T^{-2c_{5}+1/2}}{2}\right) +C(\ell T^{-1})^{1-2c_{5}} \\
&\leq &C(\ell T^{-1})^{1-2c_{5}},
\end{eqnarray*}%
which shows the claim of the lemma.\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L5a} Conditional on $\mathcal{D}_{4,T}$, for any finite constant $%
C_{6}$ and any\ $c_{6}\in (1/3,1/2)$ we have:%
\begin{equation*}
\mathrm{P}^{\ast }\left( \left \vert \frac{T^{1/2}(\hat{\theta}_{i,j}^{b}-%
\hat{\theta}_{i,j})}{\hat{s}_{i,j}^{b}}-\frac{(m\ell )^{-1/2}\sum_{t\leq
m\ell }e_{i,j,t}^{b}}{s_{i,j}}\right \vert \geq C_{6}\ell
^{c_{6}}T^{-2c_{6}+1/2}\right) \leq C(\ell T^{-1})^{1-2c_{6}}.
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} Applying (\ref{P_B_L5_7}) and (\ref{P_B_L5_8})
with $c_{5}=c_{6}$, we obtain 
\begin{eqnarray}
&&\mathrm{P}^{\ast }\left( \left \vert \left( \frac{1}{\hat{s}_{i,j}^{b}}-%
\frac{1}{s_{i,j}}\right) (m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{i,j,t}^{b}\right \vert \geq \frac{C_{6}\ell ^{c_{6}}T^{-2c_{6}+1/2}}{2}%
\right)  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \vert (m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{i,j,t}^{b}\right \vert \left \vert \frac{\hat{s}_{i,j}^{b}}{s_{i,j}}%
-1\right \vert \geq \frac{C_{6}s_{i,j}\ell ^{c_{6}}T^{-2c_{6}+1/2}}{2}%
\right) +C(\ell T^{-1})^{1-2c_{6}}  \notag \\
&\leq &\mathrm{P}^{\ast }\left( \left \vert (m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{i,j,t}^{b}\right \vert \geq \frac{C_{6}s_{i,j}T^{-c_{6}+1/2}}{2}\right)
+C(\ell T^{-1})^{1-2c_{6}}.  \label{P_B_L5a_1}
\end{eqnarray}%
Since\ $\mathrm{Var}^{\ast }((m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{i,j,t}^{b})\leq C$ under $\mathcal{D}_{4,T}$, using Markov's inequality
we get%
\begin{equation*}
\mathrm{P}^{\ast }\left( \left \vert (m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{i,j,t}^{b}\right \vert \geq \frac{C_{6}s_{i,j}T^{-c_{6}+1/2}}{2}\right)
\leq CT^{-1+2c_{6}},
\end{equation*}%
which along with (\ref{P_B_L5a_1}) shows that 
\begin{equation}
\mathrm{P}^{\ast }\left( \left \vert \left( \frac{1}{\hat{s}_{i,j}^{b}}-%
\frac{1}{s_{i,j}}\right) (m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{i,j,t}^{b}\right \vert \geq \frac{C_{6}\ell ^{c_{6}}T^{-2c_{6}+1/2}}{2}%
\right) \leq C(\ell T^{-1})^{1-2c_{6}}.  \label{P_B_L5a_2}
\end{equation}%
The claim of the lemma follows from Lemma \ref{B_L5} (with $C_{5}=C_{6}$ and 
$c_{5}=c_{6}$) and (\ref{P_B_L5a_2}).\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L6}\ Let $e_{t}^{b}\equiv (e_{i,t}^{b})_{i\leq d}$ where $%
e_{i,t}^{b}\equiv (e_{i,j,t}^{b})_{j=1,2}$.\ Conditional on $\mathcal{D}%
_{4,T}$,\ there exists a random vector\ $\mathcal{N}_{d}\sim N(0,I_{2d})$
independent of the data such that for any finite constant $C_{7}$:%
\begin{equation*}
\mathrm{P}^{\ast }\left( \left \Vert (m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{t}^{b}-(\Omega _{T}^{\ast })^{1/2}\mathcal{N}_{d}\right \Vert \geq
C_{7}\log (T)^{-2/3}\right) \leq C\log (T)^{5/2}(\ell T^{-1})^{1/2},
\end{equation*}%
where $(\Omega _{T}^{\ast })^{1/2}\equiv \mathrm{Var}^{\ast
}(T^{-1/2}\sum_{t\leq T}e_{t}^{b})$.
\end{lemma}

\noindent \textsc{Proof.} Since $(m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{t}^{b}=\sum_{j\leq m}(m\ell )^{-1/2}\sum_{l\leq \ell }e_{\ell
(j-1)+l}^{b}$ and $(m\ell )^{-1/2}\sum_{l\leq \ell }e_{\ell (j-1)+l}^{b}$ is
independent across $j$, we shall use Yurinskii's coupling to show the claim
of the lemma.\ Conditional on $\mathcal{D}_{4,T}$,\ we have 
\begin{equation*}
\mathrm{E}^{\ast }\left[ \left \Vert \sum_{l\leq \ell }(\tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b}-\mathrm{E}^{\ast }\left[ \tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b}\right] )\right \Vert ^{3}\right] \leq C%
\mathrm{E}^{\ast }\left[ \left \Vert \sum_{l\leq \ell }\tilde{R}%
_{-i,l}^{b}\varepsilon _{i,l}^{b}\right \Vert ^{3}\right] \leq C\log
(T)^{1/2}\ell ^{3/2}.
\end{equation*}%
This, along with the Cauchy-Schwarz inequality, implies that%
\begin{equation}
\sum_{j\leq m}\mathrm{E}^{\ast }\left[ \left \Vert (m\ell
)^{-1/2}\sum_{l\leq \ell }e_{\ell (j-1)+l}^{b}\right \Vert ^{3}\right] \leq
C\log (T)^{1/2}m^{-1/2},  \label{P_B_L6_1}
\end{equation}%
conditional on $\mathcal{D}_{4,T}$. Therefore, by\ Yurinskii's coupling
(see, Theorem 10 in Section 4 of \cite{pollardbook}), there exists a random
vector\ $\mathcal{N}_{d}\sim N(0,I_{2d})$ such that%
\begin{equation}
\mathrm{P}^{\ast }\left( \left \Vert (m\ell )^{-1/2}\sum_{t\leq m\ell
}e_{t}^{b}-(\Omega _{T}^{\ast })^{1/2}\mathcal{N}_{d}\right \Vert \geq
C_{7}\log (T)^{-2/3}\right) \leq C\log (T)^{5/2}(\ell T^{-1})^{1/2}
\label{P_B_L6_2}
\end{equation}%
which establishes the claim of the lemma.\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{B_L6b}\ Recall that\ $\tilde{M}_{i}^{\ast }\equiv \left \Vert (\ell
_{d,i}^{\top }\otimes \mathrm{diag}(s_{i,1}^{-1},s_{i,2}^{-1}))(\Omega
_{T}^{\ast })^{1/2}\mathcal{N}_{d}\right \Vert _{\infty }$. Conditional on $%
\mathcal{D}_{4,T}$, we have 
\begin{equation*}
\sup_{x\in \mathbb{R}}\left \vert \mathrm{P}^{\ast }\left( \max_{i\leq d}%
\tilde{M}_{i}^{\ast }\leq x\right) -\mathrm{P}\left( \max_{i\leq d}\tilde{M}%
_{i}\leq x\right) \right \vert \leq C\log (T)^{5/12}(\ell ^{2}T^{-1+2/\tilde{%
r}}+\ell ^{-1})^{1/3}.
\end{equation*}
\end{lemma}

\noindent \textsc{Proof.} Let $\xi _{i,j}$ denote the $j$-th entry of $(\ell
_{d,i}^{\top }\otimes \mathrm{diag}(s_{i,1}^{-1},s_{i,2}^{-1}))\Omega
_{d}^{1/2}\mathcal{N}_{d}$ for any $i\leq d$ and $j=1,2$. Then $\xi _{i,j}$
is normally distributed with mean zero and variance $\Omega
_{d,i}(j,j)s_{i,j}^{-2}$, where $\Omega _{d,i}(j,j)$\ denotes the $j$-th
diagonal entry of $\Omega _{d,i}$. It is clear that $\max_{i\leq d}\tilde{M}%
_{i}=\max_{i\leq d}\max_{j=1,2}\left \vert \xi _{i,j}\right \vert $. By
Assumption \ref{A2}(i), (\ref{P_I_L1_15b}), (\ref{P_I_L1_18}), (\ref%
{P_I_L3_5}) and (\ref{P_I_L1_5}),%
\begin{equation}
C^{-1}\leq \Omega _{d,i}(j,j)s_{i,j}^{-2}\leq C,  \label{P_B_L6b_1}
\end{equation}%
for any $i\leq d$ and $j=1,2$. Moreover, by (\ref{P_B_L6b_1}) and Gaussian
maximum inequality 
\begin{equation}
\mathrm{E}\left[ \max_{i\leq d}\tilde{M}_{i}\right] =\mathrm{E}\left[
\max_{i\leq d}\max_{j=1,2}\left \vert \xi _{i,j}\right \vert \right] \leq
C\log (d)^{1/2}.  \label{P_B_L6b_2}
\end{equation}%
For any $i,i^{\prime }\leq d$, we have%
\begin{eqnarray}
&&\left \Vert (\ell _{d,i}^{\top }\otimes \mathrm{diag}%
(s_{i,1}^{-1},s_{i,2}^{-1}))(\Omega _{T}^{\ast }-\Omega _{d})(\ell
_{d,i^{\prime }}\otimes \mathrm{diag}(s_{i^{\prime },1}^{-1},s_{i^{\prime
},2}^{-1}))\right \Vert  \notag \\
&\leq &\frac{\left \Vert \Omega _{T}^{\ast }-\Omega _{d}\right \Vert }{%
s_{i,1}s_{i,2}s_{i^{\prime },1}s_{i^{\prime },2}}\leq C\log (T)^{1/2}(\ell
^{2}T^{-1+2/\tilde{r}}+\ell ^{-1}),  \label{P_B_L6b_3}
\end{eqnarray}%
conditional on $\mathcal{D}_{4,T}$. Under (\ref{P_B_L6b_1}), (\ref{P_B_L6b_2}%
) and (\ref{P_B_L6b_3}), the lemma's claim follows directly from Theorem 2
in \cite{chern015comparison} with $\Delta \leq C\log (T)^{1/2}(\ell
^{2}T^{-1+2/\tilde{r}}+\ell ^{-1})$, $p=4d$ and $a_{p}=C\log (d)^{1/2}$ as
specified in the theorem.\hfill $Q.E.D.$

\bigskip

\begin{lemma}
\label{Para_Anti}\ Suppose that\ Assumptions \ref{A1}(i, ii) hold. Then for
any proper subset\ $\mathcal{S}\ $of $\mathcal{M}_{d}$\ and any $\varepsilon
\in (0,1)$,%
\begin{equation}
\sup_{u\in \mathbb{R}}\mathrm{P}\left( \left \vert \max_{i\notin \mathcal{S}}%
\tilde{M}_{i}-u\right \vert \leq \varepsilon \right) \leq C\varepsilon
(1+\log (C/\varepsilon )^{1/2}).  \label{Para_Anti_1}
\end{equation}
\end{lemma}

\noindent \textsc{Proof.} By (\ref{P_B_L6b_1}), we can apply Theorem 3(ii)
of \cite{chern015comparison} to obtain 
\begin{equation*}
\sup_{u\in \mathbb{R}}\mathrm{P}\left( \left \vert \max_{i\notin \mathcal{S}}%
\tilde{M}_{i}-u\right \vert \leq \varepsilon \right) \leq C\varepsilon
\left( \mathrm{E}\left[ \max_{i\notin \mathcal{S}}\tilde{M}_{i}\right] +\log
(C\varepsilon ^{-1})^{1/2}\right) ,
\end{equation*}%
for any $\varepsilon >0$, which together with (\ref{P_B_L6b_2}) shows (\ref%
{Para_Anti_1}).\hfill $Q.E.D.$

